Contrastive Knowledge-Augmented Meta-Learning for Few-Shot Classification

Model agnostic meta-learning algorithms aim to infer priors from several observed tasks that can then be used to adapt to a new task with few examples. Given the inherent diversity of tasks arising in existing benchmarks, recent methods use separate, learnable structure, such as hierarchies or graphs, for enabling task-specific adaptation of the prior. While these approaches have produced significantly better meta learners, our goal is to improve their performance when the heterogeneous task distribution contains challenging distribution shifts and semantic disparities. To this end, we introduce CAML (Contrastive Knowledge-Augmented Meta Learning), a novel approach for knowledge-enhanced few-shot learning that evolves a knowledge graph to effectively encode historical experience, and employs a contrastive distillation strategy to leverage the encoded knowledge for task-aware modulation of the base learner. Using standard benchmarks, we evaluate the performance of CAML in different few-shot learning scenarios. In addition to the standard few-shot task adaptation, we also consider the more challenging multi-domain task adaptation and few-shot dataset generalization settings in our empirical studies. Our results shows that CAML consistently outperforms best known approaches and achieves improved generalization.

==> CAML - Arxiv/sections/approach.tex <==
In this section, we present our approach for task-aware modulation in MAML.
% While our approach belongs to the family of structure-aware learning approaches such as ARML~\citep{yao2020automated} and HSML~\citep{yao2019hierarchically}, it fundamentally differs in the way the meta knowledge graph is constructed and the task representations are generated. 

\subsection*{Step 1: Prototype Graph Generation}
Conventionally, feature extractors are used to embed data in low-dimensional latent spaces, where the different classes are easily separable. In task-aware modulation, our goal is to obtain such representations for different few-shot tasks, such that two tasks that are similar in the latent space can use the same task network initialization for effective adaptation. Following the notations introduced in the previous section, each $k-$shot $N-$way training episode $\mathcal{T}_i^{tr}$ is comprised of support and query sets $(\mathcal{S}_{\mathcal{T}_i^{tr}} \mathcal{Q}_{\mathcal{T}_i^{tr}})$, wherein there are $k$ samples in each of the $N$ classes randomly selected from $\mathcal{C}^{tr}$. Since effective task encoding is essential for suitably modulating the initialization of the task network (see Figure \ref{fig:overview}), \name~begins by constructing a prototype-based graph \citep{yao2020automated} with the image embeddings. 

Formally, given the support set $\mathcal{S}_{\mathcal{T}_i^{tr}} \coloneqq \{(\mathrm{x}_j, \mathrm{y}_j), \forall j \in [1, \cdots, kN]\}$ for a training episode, we compute embeddings for each image $\mathrm{x}_j$ in the task using an embedding function. 
While a variety of design choices can be adopted for this, we implement the embedding function using a ResNet-18 architecture.
Given that these embeddings are used to only perform the modulation (\textit{i.e.}, the task network does not utilize these embeddings), even a shallow CNN network can be used. Using the sample-level embeddings, we then compute the prototype vector for each class $n \in [1, \cdots, N]$ by taking the average of the embeddings:
\begin{equation} \label{eq:proto_nodes}
    \mathrm{v}^n_i = \frac{1}{k} \sum_{\substack{(\mathrm{x}_j, y_j) \in \mathcal{S}_{\mathcal{T}_i^{tr}} \\ y_j = n}} \mathcal{B}(\mathrm{x}_j),
\end{equation} where $\mathcal{B}$ denotes the feature extractor that projects an image $\mathrm{x}_j$ into $\mathbb{R}^d$. Given the sensitivity of few-shot learning methods to the limited number of examples, operating on the prototype representations reduces the effect of atypical samples. While the prototype graph representation is used to both optimize the knowledge-aware task encoding and to update the meta knowledge graph, for the final task encoding, we adopt an unweighted average of node embeddings from the prototype graph.
\begin{equation}\label{eq:task_rep_vec}
    \mathrm{z}_i = \mathrm{\Psi}(\mathcal{S}_{\mathcal{T}_i^{tr}}) =  \frac{1}{N} \sum_n \mathrm{v}_i^n
\end{equation}

Node embeddings with high class separability and infused prior knowledge enables the use of such simple feature aggregation strategies in contrast to  state-of-the-art approaches such as ARML~\citep{yao2020automated} and HSML~\citep{yao2019hierarchically}, which require sophisticated aggregation strategies (e.g., RNN autoencoders) for effective task-aware modulation. 

% This is in contrast to state-of-the-art approaches such as ARML~\citep{yao2020automated} and HSML~\citep{yao2019hierarchically}, which require sophisticated feature aggregation strategies (e.g., RNN autoencoders) for effective task-aware modulation. 


% Edges in the prototype graph are a learnable function of the node embeddings, as we will discuss in the next step.

\subsection*{Step 2: Knowledge-Enhanced Task Encoding}
\label{sec:kd}
The desideratum of an ideal embedding function in task-aware modulation is to produce expressive task representations that capture the complexity of a given task. While this embedding function can be directly optimized with the goal of improving the adaptation performance with validation tasks, as done by MuMo-MAML~\citep{vuorio2019multimodal}, we propose to leverage historical experience (that evolves as we observe more training episodes) to enrich the task encoding. To this end, we adopt a meta knowledge graph structure to encode the historical experience and propose a novel contrastive distillation strategy to produce knowledge-enhanced task encodings. Note that existing structured meta-learning algorithms update the meta knowledge structure (a hierarchy or a graph) directly using gradients from the meta update step, which limits its ability to learn class-specific characteristics from the task at hand. Instead, in our approach, we do not allow gradients to directly alter the meta knowledge graph (see Figure \ref{fig:overview}), but employ an exponential moving average update based on the current task representations. As we will show in our experiments, this improved encoding of the historical experience leads to significantly improved few-shot generalization, particularly under challenging shifts.

Formally, denoting the knowledge graph for encoding experience as $\mathcal{M}$ with randomly initialized node features $\mathcal{H}_{\mathcal{M}} = \{\mathrm{h}_j\}, j = 1, \cdots, M$ and edges $\mathcal{E}_{\mathcal{M}}$, we will now describe our knowledge-aware task encoding process. Using the prototype graph from the previous step, $\mathcal{G}_i = (\mathcal{V}_i, \mathcal{E}_i)$, we perform a contrastive distillation from the meta knowledge graph $\mathcal{M}$. While the node features of the prototype graph are obtained using the embedding function $\mathcal{B}$ (as described in Step 1), those in the meta knowledge graph persist across episodes and are computed using a combination of neural message passing and an exponential moving average, to be described in Step 4. The edges in both these graphs are parameterized as a function of the absolute difference of the corresponding node features. For example, for any two nodes with features $\mathrm{a}$ and $\mathrm{b}$, $Edge(\mathrm{a},\mathrm{b}) = \sigma(\mathrm{U}^T|\mathrm{a} - \mathrm{b}|)$, where $\mathrm{U} \in \mathbb{R}^{d\times 1}$ denotes the learnable parameters and $\sigma$ is the sigmoid function. Note that for all pairs of nodes within a graph we learn a common weight matrix $U$.

In order to extract information for an episode $\mathcal{T}_i$ from historical experience, we construct a super-graph comprising nodes from both $\mathcal{G}_i$ and $\mathcal{M}$. The cross-edges between the two graphs are computed as the softmax of the set of negative Euclidean distances between all the pairs (no learnable parameters). For a pair $\mathrm{v}_i^n$ from $\mathcal{V}_i$ and $\mathrm{h}_j$ from $\mathcal{M}$,
%$$
\begin{equation}\label{eq:cross-edge}
Edge(\mathrm{v}_i^n, \mathrm{h}_j) = \frac{\exp(-\|\mathrm{v}_i^n - \mathrm{h}_j\|_2^2/\gamma)}{\sum_{\bar{n}, \bar{j}}\exp(-\|\mathrm{v}_i^{\bar{n}} - \mathrm{h}_{\bar{j}}\|_2/\gamma)}.
\end{equation}
%$$

In our implementation, we set $\gamma = 8$. In order to effectively balance between knowledge-enhanced representations and the native representations from the embedding function, we propose a contrastive learning strategy inspired by several existing self-supervised learning approaches such as SimCLR and InfoNCE~\citep{simclr,infonce}. 
% Inspired the SimCLR objective, we propose defining a positive pair  
% $$
% \mathcal{L}_{\text{SimCLR}} = - \mathbb{E} \bigg[ \log \frac{\mathsf{sim}(\mathrm{z},\mathrm{\hat{z}})}{\sum_{\mathrm{z}^{\prime},\mathrm{\hat{z}}^{\prime}} exp(\mathsf{sim}(\mathrm{z}^{\prime},\mathrm{\hat{z}}^{\prime})/\tau}\bigg],
% $$where the numerator indicates the similarity between a positive pair, the denominator corresponds to the set of negative pairs, and $f$ is a similarity function (e.g., cosine similarity). 
Here, we consider the positive pair to be the task encodings from the original prototype representations and the knowledge-enhanced prototype representations obtained via neural message passing on the super-graph. On the other hand, the negatives correspond to the node pairs from $\mathcal{G}_i$, which indicate the level of class separability in the prototype graph. This objective $ \mathcal{L}_{CKD}(\mathcal{T}_i)$ can be expressed as:
\begin{equation}\label{eq:CKD}
- \mathbb{E}\bigg[\log \frac{\exp(\texttt{sim}(\mathrm{z}_i,\hat{\mathrm{z}}_i))}{\exp(\texttt{sim}(\mathrm{z}_i,\hat{\mathrm{z}}_i)) + \sum \exp(\texttt{sim}(\mathrm{v}_i^m, \mathrm{v}_i^n))} \bigg].
\end{equation}Here, $\hat{\mathrm{z}}_i = \mathrm{\Psi}[NMP(\mathcal{G}_i,\mathcal{M})]$ indicates the knowledge-enhanced task representations obtained by first performing neural message passing (NMP) on the super-graph (similar to~\citep{yao2020automated}) and then subsequently averaging the updated prototype node representations $\hat{\mathrm{v}}_i^n$. Note that, when performing neural message passing to obtain knowledge-
enhanced task representations, we do not allow the node features in the meta knowledge graph $\mathrm{h}_j$ to be changed, and only the prototype representations are updated. Furthermore, the similarity function $\texttt{sim}$ is implemented using the cosine similarity. In effect, this attempts to modify the embedding function such that the task encoding is consistent with the historical experience while also maximizing the inter-class separability, thereby producing highly effective task representations. 

\subsection*{Step 3: Task-Specific Modulation}
The next step of our approach is to utilize the knowledge-enhanced task representations for inferring a task-specific meta initialization. The inductive biases from the historical knowledge can enable rapid adaptation of the global meta-model to a novel task. To this end, the task representation $\mathrm{z}_i$ is used to implement the following modulation function on the global task network initialization $\theta_{0}$:
\begin{equation} \label{eq:modulation}
    \theta_{0i} = \mathrm{\Gamma}(\theta_0) = \sigma(\mathbf{W}_g\mathrm{z}_i + \mathrm{b}_g) \circ \theta_0,
\end{equation}where $\mathbf{W}_g,\mathrm{b}_g$ are learnable parameters. Using a gradient-through-gradient optimization, one can then refine the task-specific initialization $\theta_{0i}$. We incorporate our distillation objective from step 2 into this task-aware modulation process from MuMo-MAML:
\begin{equation}
\label{eq:proposed}
    \min_{\bar{\theta}, \Omega} \sum_{i=1}^R \mathcal{L}(f_{\mathrm{\Gamma}(\bar{\theta}) - \alpha \nabla_{\theta} \mathcal{L}(\theta; \mathcal{S}_{\mathcal{T}^{tr}_i})\lvert_{\theta=\mathrm{\Gamma}(\bar{\theta})}}; \mathcal{Q}_{\mathcal{T}^{tr}_i}) + 
    \\ \lambda \mathcal{L}_{CKD}(\mathcal{T}_i).
\end{equation} Here, $\Omega$ corresponds to the parameters of feature extractor $\mathcal{B}$, NMP network and modulation function $\Gamma$. The hyper-parameter $\lambda$ controls the influence of the contrastive distillation term in the overall objective.

\subsection*{Step 4: Meta Knowledge Graph Update}
The final step in \name~is to evolve the meta knowledge graph $\mathcal{M}$ with the current task information. As described earlier, by not allowing gradients from the meta update step to alter node features $\mathcal{H}_{\mathcal{M}}$, we are able to better control the historical experience encoded in $\mathcal{M}$. More specifically, using the dataset $\mathcal{T}^{tr}_i$ for each $i$ in parallel, we update the node features $\mathrm{h}_j \in \mathcal{H}_{\mathcal{M}}$ using neural message passing on the super-graph to obtain $\hat{\mathrm{h}}^i_j$. In contrast to the distillation loss computation, during this NMP, we do not allow the prototype node features to be changed and update only the node features of $\mathcal{M}$. 
Note that, for both the prototype and the knowledge graphs, we use the edges inferred after the meta update in Step~3. Let $\hat{\mathrm{h}}_j$ denote the average of all the $\hat{\mathrm{h}}^i_j$. Finally, we employ an exponential moving average update of the node features of the meta knowledge graph via $\mathrm{h}_j = \alpha \hat{\mathrm{h}}_j + (1 - \alpha) \mathrm{h}_j$, where the hyper-parameter $\alpha$ controls the amount of history retained from previous episodes.

% \RestyleAlgo{boxruled}
    % \begin{center}
    
\begin{algorithm2e}[t]
    \SetAlgoLined
    \DontPrintSemicolon
    \caption{~Training of \name}\label{algo1}
    
	\textbf{Input}: $p^{tr}(\mathcal{T})$ Distribution over training tasks, hyper-parameters $\alpha,\lambda$ \;
	
	\textbf{Learnable Parameters}: Embedding network $\mathcal{B}$, task network $f(\theta_0)$, modulation parameters $\mathrm{\Gamma}$, meta knowledge graph $\mathcal{M}$, NMP network\;
	
	\textbf{Initialization}: Randomly initialize parameters $\theta_{0}$, $\mathcal{B}$, $\mathcal{M}$, and NMP network
	 \;
    
    \While{not done}{
        Sample a batch of tasks $\mathcal{T}_i^{tr} \sim p^{tr}(\mathcal{T})$;
            
            //meta-train // \\
            \For {each $\mathcal{T}_i^{tr}$}{
                Sample $\mathcal{S}_{\mathcal{T}_i^{tr}}$ and$ \mathcal{Q}_{\mathcal{T}_i^{tr}}$ from $\mathcal{T}_i^{tr}$\;
                
                
                Randomly initialize learnable edges of $\mathcal{M}$ \;
                
                Compute the prototype vectors $\mathcal{V}_i$ following equation \eqref{eq:proto_nodes} \;
                
                 Construct prototype graph $\mathcal{G}_i$ with learnable edges \;
                
                Construct the task representation vector $\mathrm{z}_i$ following equation \eqref{eq:task_rep_vec}\;
                
                
                Compute the contrastive objective $\mathcal{L}_{CKD}(\mathcal{T}_i)$ following equation \eqref{eq:CKD} \;

                Perform task-aware modulation using $\mathrm{z}_i$ following equation \eqref{eq:modulation} \;
                
             Update 
            $\theta^{*}_0 = \theta_0  - \alpha \nabla_{\theta} \mathcal{L}(\theta; \mathcal{S}_{\mathcal{T}^{tr}_i})$ \;
            }
            //meta-update// \\
            Minimize the objective in \eqref{eq:proposed} and update $\theta_0$, $\mathcal{B}$, $\mathrm{\Gamma}$, edge weights of $\mathcal{M}$, and NMP network\;
            
            \For {each $\mathcal{T}_i^{tr}$}{
            Obtain $\hat{\mathcal{H}}^i_{\mathcal{M}}$ with $\mathcal{G}_i$ using the strategy in Step 4 of Section 4. 
            }
            Update $\mathcal{M}$ using $\hat{\mathcal{H}}_{\mathcal{M}}$ averaged over $\mathcal{T}_i^{tr}$
    }
		 
	
\end{algorithm2e}
% \end{center}
    
% \RestyleAlgo{boxruled}
%     \begin{center}
%     \begin{algorithm}[t]
    
% 	\KwIn{$p^{te}(\mathcal{T})$ Distribution over testing tasks, 
% 	 Embedding network $\mathcal{B}$, task network $f(\theta_0)$, modulation parameters $\mathrm{\Gamma}$}
% 	\KwOut{Adaptation performance}
    
%         Sample a batch of tasks $\mathcal{T}_i^{te} \sim p^{te}(\mathcal{T})$;
            
%             \For {each $\mathcal{T}_i^{te}$}{
%                 Sample $\mathcal{S}_{\mathcal{T}_i^{te}}$ and$ \mathcal{Q}_{\mathcal{T}_i^{te}}$ from $\mathcal{T}_i^{te}$\;
                
                
%                 Compute the prototype vectors $\mathcal{V}_i$ following equation \eqref{eq:proto_nodes}.
                
%                 Construct the task representation vector $\mathrm{z}_i$ following equation \eqref{eq:task_rep_vec}.\;

%                 Perform task-aware modulation using $\mathrm{z}_i$ following equation \eqref{eq:modulation}. \;
                
%              Fine-tune the task network $f(\theta_{0i})$ using the support set $ \mathcal{S}_{\mathcal{T}_i^{te}}$. \;
            
%             Evaluate performance of the fine-tuned model $f$ using the query set $\mathcal{Q}_{\mathcal{T}_i^{te}}$.
%             }
% 	\caption{~Adaptation with \name}\label{algo1}
% \end{algorithm}
% \end{center}
% n contrast, we update the knowledge structure with the information from the prototype graph using moving average based update strategy. In lieu of this, we transfer information from the prototype graph to knowledge structure utilizing neural message passing as described in \ref{}. 

%Another crucial step in METHOD is to update the knowledge strucutre with current task information. Recent structure-aware methods use gradients from the meta-update stage to update the knowledge structure. This gradient based update doesn't ensure effective capture of task information, rather focuses on minimizing the meta-update loss. I

% to the prototype graph $R_i = (C_i,\mathcal{E}_{i})$ ($\mathcal{E}_{i}$ represents edges of the prototype graph) to obtain prior knowledge enhanced prototype nodes $\hat{C_i}$. 
% \begin{equation}
%     \hat{C_i} = NMP(R_i, G),
% \end{equation} where NMP represents neural message passing stragegy employed by ARML.
% The $\hat{C_i}$ is aggregated following equation \ref{} to obtain the prior knowledge enhanced task representation $t_i \in \mathbb{R}^d$.

% To effectively distill task relevant historical information, we introduce a contrastive learning objective between the task representation $q_i$ and the prior knowledge enhanced task representaion $t_i$. More specifically, we compute the positive pair of the contrastive objective as the coscine similarity between $q_i$ and $t_i$:
% \begin{equation}
%     pos = -\sum^d l2_{normalize}(q_i)* l2_{normalize}(t_i),
% \end{equation} where $d$ is the embedding dimension of the task representation vector. The positive pair ensures that the embedding function learns class relevant prior task information from the knowledge structure. In order to enforce sufficient class separation between prototype representations, such that the embedding of different classes are farther apart, we compute a negative pair between the nodes $c_i^k$ of the prototype representation $\mathcal{C}_i$.

% \begin{equation}
% neg = -\sum_{m=1}^{K}\sum_{j=1}^{K}\sum^d(l2_{normalize}(c^j_i) * l2_{normalize}(c^m_i),
% \end{equation}

% % Furthermore, It is important to ensure that the historical information extracted by the prototype graph is novel from the feature extractor infused prior task information carried by the prototype nodes. In light of this we introduce a negative term to the contrastive loss computed as the cosine similarity between $C_i$ and $C_s = NMP(C_i, C_i)$:

% % \begin{equation}
% % neg_2 = -\sum_{m=1}^{K}\sum_{j=1}^{K}\sum^d(l2_{normalize}(c^j_i) * l2_{normalize}(cs^m_i),
% % \end{equation} 
% Using the positive and negative pair, we compute the contrastive loss as:
% \begin{equation}
%     \mathcal{L}_c = - \log \frac{pos}{neg},
% \end{equation}

% In effect, the contrastive loss ensure that the prototype representation obtained from the feature extractor carries prior task information while maintaining class separability.
% The task-relevant historical information encapsulated by the knowledge structure is distilled to the feature extractor by minimizing a contrastive loss between the task representation and the prior knowledge enhanced task representation. The prior knowledge enhanced task representation is an aggregate of the prototype graph enhanced with historical task information from the knowledge structure. Further, the knowledge structure is updated using weighted moving average update with the current task information through neural message passing. In the rest of this section, we describe the proposed approach in detail.

% In this section, we present \method, a gradient-based meta-learning approach for few-shot classification, which constructs a hierarchy of knowledge graphs to effectively represent task relationships. For a novel test task, \method~can automatically extract relevant information from the knowledge structure and appropriately tailor the meta-initialization parameters. While our approach belongs to the family of structure-aware meta-learning approaches such as ARML and HSML, it fundamentally differs by the structure utilized for modeling relationships between tasks. 

% As illustrated in Figure \ref{fig:overview}, for a given task $\mathcal{T}_i$, we construct a prototype-based graph representation~\citep{yao2020automated}, and distill the task-relevant knowledge from every level of the knowledge graph hierarchy in order to update the prototype graph with historical task information. We then use an aggregate of the original task representation and the enhanced prototype graph to tailor the global initialization parameters $\theta_0$ to effectively solve the current task. In the rest of this section, we describe the proposed approach in detail.
    
% \subsection{Representing Tasks using Prototype Graphs}
% For an input task $\mathcal{T}_i$ with training samples $(\mathrm{x}_j, \mathrm{y}_j) \in D^{tr}_i | \forall j \in [1,N^{tr}]$, we first construct a prototype-based relational graph $\mathcal{R}_i$. The nodes $\mathcal{C}_{i}$ denote the prototypes corresponding to different classes in $\mathcal{D}_i^{tr}$ and the edges $\mathcal{E}_{i}$ indicate the similarities between prototypes. Note that using the class prototypes to construct $\mathcal{R}_i$ leads to more reliable task representations. As opposed to the vector embeddings used in TAM~\citep{vuorio2019multimodal} or HSML~\citep{yao2019hierarchically}, such representations are more expressive both to capture cross-task relations as well as to retrieve relevant information from the learned knowledge structure. Following standard practice in image classification models, the prototypes are computed using features from an embedding network $\mathcal{B}$:
% \begin{equation} \label{eq:3}
% \mathrm{c}^k_{i} = \frac{1}{N^{tr}_k} \sum^{N^{tr}_k}_{j=1} \mathcal{B}(\mathrm{x}_j),
% \end{equation}where $N^{tr}_k$ denotes the number of samples in class $k$ and the embedding function $\mathcal{B}$  projects an image $\mathrm{x}_j$ into $\mathbb{R}^d$, such that samples from the same class are closer to each other.  Thus, our prototype for each class, which becomes the features for that class' node in $\mathcal{C}_i$, is the mean embedding of the images in that class.  %Using the 

% We compute edges $\mathcal{E}_{i}$ of the prototype graph based on the similarity between the node features:
% \begin{equation}
% \mathcal{E}_{i}(\mathrm{c}^j_i, \mathrm{c}^m_i) = \sigma(\|\mathrm{c}^j_i - \mathrm{c}^m_i\|^2_2),
% \label{eqn:protoedge}
% \end{equation}where $\mathrm{c}^j_i,\mathrm{c}^m_i$ are two different nodes in $\mathcal{C}_{i}$ and $\sigma$ denotes the sigmoid function. In our empirical studies, not including any additional learnable parameters in \eqref{eqn:protoedge} leads to a more stable convergence of our meta-learning algorithm.


% \subsection{Constructing Knowledge Graph Hierarchies}
% To efficiently extract prior knowledge relevant to the current task $\mathcal{T}_i$, we propose to utilize knowledge graph hierarchies. While each level in the hierarchy represents historical task priors at different complexity, each knowledge graph in a level represents different task groups at a certain complexity. Formally, we represent our proposed knowledge graph hierarchies as
% \begin{equation} \label{eq:5}
%     \Gamma = \{\mathcal{G}_{\ell}^m|\forall \ell \in [1,\ldots, L], m \in [1,\ldots, M_{\ell}]\}
% \end{equation}where $L$ denotes the total number of levels and $M_{\ell}$ represents the number of knowledge graphs in level $\ell$.

% In order to automatically infer the knowledge structure, every meta-graph $\mathcal{G}_{\ell}^m = (\mathcal{H}_{\ell}^m, \mathcal{A}_{\ell}^m)$ is initialized with learnable node features $\mathcal{H}_{\ell}^m \in \mathbb{R}^{V \times d}$, and the corresponding adjacency matrix $ \mathcal{A}_{\ell}^m \in \mathbb{R}^{V\times V}$. Here, $V$ denotes the total number of vertices for each meta-graph. Similar to the prototype graph construction, the edge weights between two vertices $\mathrm{h}_p$ and $\mathrm{h}_q$ in a meta-graph $\mathcal{G}_{\ell}^m$ can be obtained as:
% \begin{equation} \label{eq:6}
% \mathcal{A}_{\ell}^m(\mathrm{h}_p, \mathrm{h}_q) = \sigma\bigg(\mathbf{W}_{pq}^{\ell,m}(|\mathrm{h}_p - \mathrm{h}_q|) + \mathrm{b}_{pq}^{\ell,m}\bigg),
% \end{equation}where $\mathbf{W}_{pq}^{\ell,m}$ and $\mathrm{b}_{pq}^{\ell,m}$ represent learnable weights and biases. Note that the parameters, the node features, and edge functions are updated at meta-test time using $D^{ts}_i$, the (limited) labeled data used to adapt to the new task.  

% \subsection{Augmenting Task Representations via Message Passing}
% For every input task $\mathcal{T}_i$, our goal is to update the prototype graph representation by distilling task-specific knowledge from each level of the knowledge graph hierarchy. At level $\ell$, we systematically propagate information from each of the meta-graphs $\mathcal{G}_{\ell}^m$ to the prototype graph by constructing a super-graph $\mathcal{S}_i^{\ell, m}$ and then performing neural message passing to update node features $\mathcal{C}_{i}$. The vertices of the super-graph correspond to the union of vertices from $\mathcal{R}_i$ and $\mathcal{G}_{\ell}^m$, and existing edges within each of the two graphs are retained.  We also add edges between the vertices $\mathcal{C}_{i}$ of the prototype graph and the vertices $\mathcal{H}_{\ell}^m$ of the $m^{\text{th}}$ knowledge graph in level $\ell$ using a Gaussian kernel-based link function:
% \begin{equation} \label{eq:7}
%     \mathcal{Q}_i^{\ell, m}(\mathrm{c}_i^k, \mathrm{h}_p) = \frac{\exp(-\|(\mathrm{c}^k_i - \mathrm{h}_p)/\gamma\|^2_2/2)}{\sum^V_{v=1} \exp(-\|(\mathrm{c}^k_i - \mathrm{h}_v)/\gamma\|^2_2/2)}.
% \end{equation}
% where $\mathrm{h}_v, \mathrm{h}_p \in \mathcal{H}_{\ell}^m$ and $\gamma$ is a scaling factor. This process results in the super-graph, denoted as $\mathcal{S}_i^{\ell, m} = (\mathcal{C}_{i} \bigcup \mathcal{H}_{\ell}^m,  \mathcal{Q}_i^{\ell, m})$, comprising $K + V$ vertices in total.

% Following the messaging passing strategy adopted by ARML~\citep{yao2020automated}, we leverage a Graph Convolutional Network (GCN)~\citep{kipf2016semi} to distill information from the knowledge graph to update the task representation. 

% After carrying out a GCN forward pass on the super-graph, the top $K$ components of the updated feature set correspond to the prototype graph updated with prior task knowledge from $\mathcal{G}_{\ell}^m$. Using this approach, one can distill from each of the knowledge-graphs in level $\ell$ to obtain $M_{\ell}$ updated prototype graphs. Formally, for every KG in level $1$, we compute
% \begin{equation} \label{eq:8}
%     \hat{\mathcal{C}}_i^{1,m} = \texttt{GCN}(\mathcal{V}_i, \mathcal{G}_{1}^m)
% \end{equation}The resulting representations from any level $\ell$ are subsequently used to select relevant information from the next $(\ell+1)^{\text{th}}$ level in the hierarchy. Though one can employ an attention mechanism to compute relevance of a knowledge graph $n$ in level $\ell+1$ using the updated prototype representation at knowledge graph $m$ in level $\ell$, similar to the soft cluster assignment in HSML~\citep{yao2019hierarchically}, we find that a uniform attention itself is highly effective. In other words,
% \begin{equation} \label{eq:9}
%     \hat{\mathcal{C}}_i^{\ell+1,n} = \frac{1}{M_{\ell}} \sum_{m=1}^{M_{\ell}} \texttt{GCN}(\hat{\mathcal{C}}_i^{\ell,m}, \mathcal{G}_{\ell+1}^n)
% \end{equation}Through this hierarchical knowledge distillation process, our approach systematically incorporates task-relevant information at different levels of complexity. After processing information in all $L$ levels of the knowledge graph hierarchy, the final task representation for the task $\mathcal{T}_i$ is obtained by performing average pooling of all $M_L$ prototype representations in the last level.
% \begin{equation} \label{eq:10}
% \hat{C}_{i} = \frac{1}{M_L}\sum_{m=1}^{M_L} \hat{C}_{i}^{L, m}.
% \end{equation}From our empirical studies, we make the striking observation that knowledge graph hierarchies provide a powerful way to improve the expressive power of the knowledge structures in capturing cross-task relationships. Interestingly, the performance of existing approaches such as ARML declines steadily as one arbitrarily increases the number of vertices in the meta-knowledge graph. With \method~,we can either increase the depth $L$ of the hierarchy or alternately increase the number of graphs $M_{\ell}$ in any level to enhance its expressive power.

% \subsection{Task-Specific Modulation of Meta Parameters}
% The final important step of our meta-learning algorithm is to utilize the enhanced task representations for inferring task-specific meta initializations. Our implementation of this step exactly follows HSML~\citep{yao2019hierarchically} and ARML~\citep{yao2020automated}, where the task-relevant information from the hierarchy along with the original prototype graph are used to perform task-aware modulation. The inductive biases from the historical knowledge can enable rapid adaptation of the global meta-model to any task from a heterogeneous task distribution. To this end, we first aggregate $C_{i}$ and $\hat{C}_{i}$ into vector representations using two RNN-based autoencoders. The RNN aggregators create dense representations for each $\mathrm{c}_i^j \in C_{i}$ and $\hat{\mathrm{c}}_i^j \in \hat{C}_{i}$. Finally, concise task embedding vectors $\mathrm{q}_i$ and $\mathrm{t}_i$ for $C_{i}$ and $\hat{C}_{i}$ respectively are obtained by performing average pooling over all $K$ vertices.

% \begin{equation}
%     \mathrm{q}_i = \frac{1}{K}\sum_{j=1}^{K}(\Psi_q^{\text{enc}}(\mathrm{c}_i^j));  \mathrm{t}_i = \frac{1}{K}\sum_{j=1}^{K}(\Psi_t^{\text{enc}}(\hat{\mathrm{c}}_i^j))
%     \label{eq:agg}
% \end{equation}In order to train these two RNN aggregators, we also include two additional reconstruction loss terms based on both the encoder-decoder networks:
% \begin{align}
%     \mathcal{L}_q &= \sum_{j}\|\mathrm{c}_{i}^j - \Psi^{\text{dec}}_q(\Psi^{\text{enc}}_q(\mathrm{c}_i^j))\|_2, \\
%     \mathcal{L}_t &= \sum_{j}\|\hat{\mathrm{c}}_{i}^j - \Psi^{\text{dec}}_t(\Psi^{\text{enc}}_t(\hat{\mathrm{c}}_i^j))\|_2.
% \end{align}Along with the parameters of knowlege graph hierarchy and the base learner, the two autoencoders are updated using the meta-test set $D_i^{ts}$. 

% The task representations $\mathrm{q}_i$ and $\mathrm{t}_i$ are used to implement the modulation function for obtaining task-specific initialization $\theta_{0i}$:
% \begin{equation} \label{eq:11}
%     \theta_{0i} = \sigma(\mathbf{W}_g(\mathrm{q}_i \oplus \mathrm{t}_i) + \mathrm{b}_g) \circ \theta_0,
% \end{equation}where $\oplus$ denotes the concatenation operation and $\mathbf{W}_g,\mathrm{b}_g$ are learnable parameters. Using a gradient-through-gradient optimization, one can then refine the task-specific initialization $\theta_{0i}$. In summary, we use the $\theta^*_{0i}$ (computed in the meta-train phase) to infer parameters of the knowledge graph hierarchy $\Gamma$, task embedding function $\mathcal{B}$, and the task aggregators using following optimization objective:
% \begin{equation} \label{eq:12}
%     \sum_{\mathcal{T}_i \in P(\mathcal{T})} \mathcal{L}(f_{\theta^*_{i}}, D_i^{ts}) + \mu_1\mathcal{L}_q + \mu_2\mathcal{L}_t,
% \end{equation}where $\mu_1, \mu_2$ are user-specified hyper-parameters.

% \RestyleAlgo{boxruled}
% \begin{minipage}{0.45\textwidth}
% \centering
%     \begin{algorithm}[H]
% 	\KwIn{$P(\tau)$ Distribution over heterogeneous tasks. 
% 	$\ell$: number of levels in hierarchical structure $\Gamma$; $M_{\ell}$ : number of knowledge graphs in level $\ell$.}
% 	\KwOut{ Learned structure $\Gamma$, embedding network $\mathcal{B}$, RNN aggregators, base learner $f(\theta_0)$}
% 	\textbf{Initialization}: Randomly initialize parameters $\theta_{0}$. parameters of $\Gamma$ and
% 	hyper-parameters $\alpha,\gamma, \mu_1, \mu_2$ \;
    
%     \While{not done do}{
%         Sample a batch of tasks $\tau_i \sim P(\tau)$;
            
%             //meta-train // \\
%             \For {each $\tau_i$}{
            
%                 Sample $D^{tr}_i$ and $D^{ts}_i$ from $\tau_i$\;
                
%                 Construct prototype graph $\mathcal{R}_i$ using \eqref{eq:3} and \eqref{eqn:protoedge}\;
                
%                 Extract knowledge from $\Gamma$ to get updated prototype representation following \eqref{eq:7}-\eqref{eq:10}\;
                
%                 Aggregate the original and the knowledge-enhanced task representation using \eqref{eq:agg}\;
            
%                  Perform task-aware modulation using \eqref{eq:11}\;
                
%              Update $\theta^{*}_0 = \theta_0 - \alpha  \nabla_{\theta_{0}} \mathcal{L}(\theta_{0};D_i^{tr})$ \;
%             }
%             //meta-update//\\
%             Update $\theta_0$, $\Gamma$, $\mathcal{E}$ and RNN aggregators to minimize the objective in \eqref{eq:12}
%     }
		 
% 	\caption{~Training of SGML}\label{algo1}
% \end{algorithm}
% \end{minipage}



==> CAML - Arxiv/sections/intro.tex <==
Learning to solve new tasks using only few-shot examples is a long-standing challenge. Meta-learning forms an important class of few-shot learning algorithms that leverages transferable knowledge priors from previously learned tasks to learn new tasks quickly. For example, the widely adopted model-agnostic meta-learning (MAML) approaches~\citep{finn2017model,yoon2018bayesian,lee2018gradient,finn2018probabilistic,finn2017meta} attempt to learn a single \textit{meta} model (or base learner) on a set of observed tasks, which is assumed to be only a few gradient descent steps away from good task-specific models. Their success hinges on the assumption that the observed tasks are realizations from a common task distribution $p(\mathcal{T})$. Despite its mathematical tractability, the premise of using a single base learner can be insufficient when $p(\mathcal{T})$ is heterogeneous, \textit{i.e.}, the degree of similarity between tasks can be vastly different~\citep{vuorio2019multimodal}. This motivates the need for a meta-model to selectively utilize knowledge from its previous experience that is the most relevant for the target task. 
%, akin to human intelligence %for machine-learned models %set of the task distribution %For example, it can contain both semantically similar (e.g. classifying sparrows and ravens) or disparate (e.g. classifying flowers and traffic signs) tasks, making the assumption of a single base learner restrictive.

In this context, task-aware modulation~\citep{vuorio2019multimodal} (MuMo-MAML) is an important principle to improve the performance of MAML on heterogeneous tasks. Conceptually, MuMo-MAML infers latent representations to characterize realizations from a heterogeneous task distribution, and modulates the base learner initialization appropriately, based on latent characteristics, to improve the adaptation performance. In a quest to improve upon MuMo-MAML, recent methods have resorted to using a separate learnable structure for encapsulating relationships across the training episodes~\citep{vuorio2019multimodal,yao2019hierarchically,yao2020automated}. This meta structure can then be leveraged when adapting to a new task by selectively utilizing knowledge from prior experience. Though these approaches have been found to outperform vanilla MuMo-MAML in few-shot adaptation tasks, they have the risk of overfitting the \textit{task encoding network} to the observed distribution of training tasks. As we demonstrate in this paper, this behavior can be particularly limiting in the more challenging (yet practical) settings of multi-domain task adaptation~\citep{peng2019moment} and few-shot dataset generalization~\citep{triantafillou2021learning}.
% they lack the ability to generalize prior experience to solve more challenging problems like multi-domain task adaptation and generalizing prior experiences to tasks sampled from novel unseen distribution.
%For example, the recent ARML (automated relational meta learning)~\citep{yao2020automated} approach evolves a meta knowledge graph for improving the encoding of tasks drawn from heterogeneous task distributions.This critical insight has led to the design of a new class of approaches that perform structured storage and retrieval of task-relevant information. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/problems.pdf}
    \caption{\textbf{Few-shot classification tasks}. Here, we formally define the different problem settings considered in this study. As we move from few-shot adaptation to few-shot dataset generalization, the problem becomes increasingly challenging and requires sophisticated task-aware modulation strategies to improve the performance of MAML.}
    \label{fig:problems}
\end{figure*}

\noindent \textbf{Proposed Work.} We introduce a new approach, Contrastive Knowledge-Augmented Meta Learning (\name), for task-aware modulation in MAML with the goal of advancing the generalization capabilities of meta-learners. At its core, CAML utilizes prototype graphs to represent a few-shot task and leverages an external meta knowledge structure to construct task embeddings, which are subsequently used to modulate the base learner parameters. CAML constructs the meta knowledge structure from the observed tasks similar to state-of-the-art methods~\citep{yao2020automated}, albeit with the following key differences: (i) CAML uses a contrastive knowledge distillation strategy to systematically infuse prior knowledge directly into the image embedding module, which leads to richer task representations and eliminates the need to perform knowledge extraction during inference time; (ii) Through the improved image embeddings, CAML enables a task encoding scheme without any learnable parameters (average pooling) to construct task representations; in contrast, state-of-the-art approaches rely on complex task encoding modules; (iii) CAML employs a moving average-based update strategy for the knowledge structure, which leads to improved encoding of the prior experience compared to existing approaches~\citep{yao2019hierarchically,yao2020automated}. 
% We find that these three components are critical to improving the generalization of task-aware modulation approaches in few-shot learning.

We evaluate \name~and compare to other few-shot learning methods using three experimental settings (see Figure \ref{fig:problems}): (i) the standard few-shot adaptation setting, where the goal is to adapt to novel classes within the observed datasets; (ii) multi-domain adaptation, where the goal is to learn priors using data sampled from different domains and adapt to unseen test tasks sampled from any of the observed domains; and (iii) few-shot dataset generalization, where the test tasks are sampled from novel unseen datasets that are not observed during training. We make an interesting finding that, even without using the knowledge structure for inference, \name is able to produce highly effective task-specific initializations. While \name~is very competitive in the standard task adaptation setting, in the multi-domain setting, its benefits become even more apparent, and we observe larger performance gains ($2\% - 3\%$ for both $1-$shot and $5-$shot training). Finally, in the most challenging dataset generalization setting, we find that \name~significantly outperforms the state-of-the-art structure-aware learning method (ARML~\citep{yao2020automated}), with gains as high as $~5\%$ and $~10\%$ in $1$- and $5$-shot training respectively.
%, thus standing testimony to the effectiveness of our knowledge distillation process.
% improves upon popular meta-learning approaches in the few-shot task adaptation setting ($0.7\%$ on average)


% As expected, the success of this approach hinges on the ability of the learned task representations to encapsulate all relationships between the large number of observed tasks used for MAML training (several tens of thousands), and this is known to be very challenging in practice. 
% which demonstrates the ability of \name to generalize prior experiences to unseen tasks in the data generalization scenario.
% Our contributions are as follows:
% \begin{itemize}
%     \item We propose a new structure aware meta-learning approach, which distills prior task information from the knowledge structure to the embedding function.
%     % \item We empirically showcase the utility of our more expressive knowledge structure by obtaining average performance gains of $\sim2\%$ over state-of-the-art structured meta-learning approaches.
%     \item We study the new scenario of out-of-distribution few-shot learning, where the model is evaluated on tasks from unseen datasets, and show that our method's superior inductive bias improves performance by  $~3\%$ on novel unseen tasks when compared with state-of-the-art framework ARML.   
% \end{itemize}

% On the contrary, during test time, it is crucial for meta-learning methods to utilize prior experience to solve tasks sampled from unseen distributions, breaking the \textit{iid} assumption.

% In real world scenario in addition to training tasks sampled from heterogeneous datasets the test-time tasks are sampled from previously unseen datasets
% However, these methods lack the ability to generalize prior experience to tasks sampled from unseen distributions. This could be attributed to the reliance on the gradients from the base learners performance on the test tasks to learn prior task experiences. Such gradient based knowledge update does not guarantee encapsulation of class specific information from the tasks. Utilizing such non-specific information for modulating the initial parameters of the base learner becomes challenging and requires sophisticated task aggregation strategies(RNN).

% In this paper we propose a framework that, during training stage, distills prior task knowledge encapsulated by the knowledge structure into the embedding function using a contrastive objective. With the prior task knowledge the embedding function can generate image embeddings infused with relevant prior information. Such embeddings eliminate the need for complex task aggregation and could adopt a simple averaging mechanism to obtain task representations. With the prior knowledge fused into the image embeddings, our proposed method does not require task specific knowledge extraction from the knowledge structure during inference time. Diverging from gradient based update of the prior knowledge structure utilized by ARML, we adopt a weighted average method to update  Neural Message Passing(NMP) to update the knowledge structure with current task information. The prototype graph employs 
% Our extensive experimentation demonstrate that the  

% However, in comparison to  HSML, ARML lacks the ability to organize knowledge at different levels (coarse and fine-grained), which we find to be very important for improving the expressive power of the knowledge structure.
    
% In this paper, we propose \method, which unifies the strengths of these different families of structured meta-learning methods. \method~adopts a graph-based learning framework, similar to ARML, but also organizes task-relevant priors at different levels of complexity in the form hierarchies of knowledge graphs. More specifically, each input task is represented as a graph of class prototypes and the node features in this graph are augmented with relevant historical information from the knowledge structure through a neural message passing mechanism.  Finally, the prototype graph and the augmented prototype graph are aggregated to perform task-aware modulation of the shared base learner. Using the Meta-Dataset benchmark~\citep{triantafillou2019meta}, we carried out empirical studies to compare the proposed \method~with state-of-the-art structured meta-learning approaches, namely HSML and ARML, and we find that \method~provides significant performance gains even with highly heterogeneous tasks.


% Following ARML, a prototype-based relational graph is constructed for each class in a given task, where each vertex represents a prototype and the edges represents the relationship between the prototypes. The prototype graph is augmented by the knowledge represented in the tree of graphs by hierarchically extracting information from graphs of each level. 
% The knowledge from each graph in a given level is selectively extracted based on the information similarity between the augmented prototype graph from the previous level and the knowledge graphs.
% The augmented prototype graph represents the current task enhanced with relevant historical task knowledge. The information from the prototype graph and the augmented prototype graph is used to modulate knowledge from the current task and historical tasks to the task-specific parameters and adapt the model to the new task.

% Our contributions are as follows:
% \begin{itemize}
%     \item We propose \method, a new structured meta-learning approach, which learns a hierarchy of knowledge graphs to represent information from historical tasks and performs task-aware modulation for effective adaptation.
%     \item We empirically showcase the utility of our more expressive knowledge structure by obtaining average performance gains of $\sim2\%$ over state-of-the-art structured meta-learning approaches.
%     \item We study the new scenario of out-of-distribution few-shot learning, where the model is evaluated on tasks from unseen datasets, and show that \method's superior inductive bias improves performance by  $~3\%$ on novel unseen tasks when compared with state-of-the-art framework ARML.   
% \end{itemize}

==> CAML - Arxiv/sections/overview.tex <==


While the few-shot learning literature encompasses a wide variety of training algorithms, meta-learning is a popular choice~\citep{thrun2012learning} for both classification and reinforcement learning~\citep{nagabandi2018learning}. Existing few-shot meta-learning approaches can be broadly categorized into: 1) metric-based meta-learning frameworks~\citep{snell2017prototypical,koch2015siamese,vinyals2016matching} that learn a metric or distance function to compare different exemplars; 2) model-based approaches where meta-learning models learn to adjust the model parameters to adapt to new tasks~\citep{munkhdalai2017meta,santoro2016meta}; and 3) gradient-based model agnostic meta-learning models. In particular, our work builds upon model agnostic meta-learning (MAML)~\citep{finn2017model} formulated as follows:

\paragraph{\textbf{Model Agnostic Meta-Learning.}} Given a set of episodes, $\{\mathcal{T}^{tr}_1, \cdots, \mathcal{T}^{tr}_R\}$ comprised of support and query sets ($\mathcal{T}^{tr}_i = (\mathcal{S}_{\mathcal{T}^{tr}_i},\mathcal{Q}_{\mathcal{T}^{tr}_i})$), from the training set $\mathcal{D}^{tr}$, MAML considers the meta-learner as the initialization of a task network $f$, \textit{i.e.}, $\theta_0$, and optimizes for a well-generalized initialization $\theta_0^*$. Formally, 
\begin{align}
    \theta_0^* &= \arg \min_{\bar{\theta}} \sum_{i=1}^R \mathcal{L}(f_{\theta_i}; \mathcal{Q}_{\mathcal{T}^{tr}_i}) \\ 
    &= \arg \min_{\bar{\theta}} \sum_{i=1}^R \mathcal{L}(f_{\bar{\theta} - \alpha \nabla_{\theta} \mathcal{L}(\theta; \mathcal{S}_{\mathcal{T}^{tr}_i})\lvert_{\theta=\bar{\theta}}}; \mathcal{Q}_{\mathcal{T}^{tr}_i}),
    \label{eq:meta}
\end{align}where the task-specific initialization $\theta_i$ is obtained using a gradient step from the meta-initialization $\theta_0$. Note, the notation $\bar{\theta}$ refers to the variables used during the optimization of this bi-level objective function. Here, $\mathcal{L}(\theta; \mathcal{S}_{\mathcal{T}^{tr}_i})$ is implemented as the cross entropy loss $\sum_{(\mathrm{x}, \mathrm{y})\in \mathcal{S}_{\mathcal{T}^{tr}_i}} \log P(\mathrm{y} | \mathrm{x}, f_{\theta})$.
%(or mean sqaured  error in regression) 

\vspace{0.1in}
\noindent \textbf{\textbf{Task-Aware Modulation.}} When the tasks used for meta-learning are sampled from a heterogeneous task distribution, inferring a common parameter initialization $\theta_0$ for all tasks can be fundamentally restrictive. Hence, task-aware modulation~\citep{vuorio2019multimodal} is a more effective formulation that aims at building a meta-learner which can generalize on heterogeneous task distributions through a set of latent parameters representing task-specific characteristics. For example, MuMo-MAML first uses a task encoder to encode the training episode for a given task into a task embedding vector $\mathrm{v}_i$. The task embedding is then used to obtain modulation vectors that are applied to the global initial parameters $\theta_0$ thereby producing task-aware initialization $\theta_{0i}$. Extending the MAML formulation in \eqref{eq:meta}, the task-aware modulation can be carried out using the support set in the training episode $\mathcal{S}_{\mathcal{T}^{tr}_i}$ and the updated initialization $\theta_{0i}$ is used to perform the meta-optimization.

While task-specific initialization can lead to improved generalization on heterogeneous tasks, its effectiveness relies on the ability of the task embeddings to encapsulate all relationships between the large number of observed tasks and thus performing similar parameter modulation for related tasks. Since it is challenging to learn such expressive embeddings, more recent approaches have resorted to storage and retrieval of task-relevant information from historical experience, in order to better balance generalization and customization (task-aware modulation)~\citep{yao2019hierarchically,yao2020automated}. For example, the recently proposed hierarchically structured meta learning (HSML) and automated relational meta-learning (ARML) approaches~\citep{yao2020automated} use an external meta knowledge structure to assist the task encoding process. By adopting these knowledge-enhanced representations coupled with a sophisticated RNN-based task encoder, these approaches are known to outperform MAML and MuMo-MAML in the standard, few-shot task adaptation setting.

\vspace{0.1in}
\noindent \textbf{\textbf{Our Approach.}} In this paper, our goal is to improve the performance of task-aware modulation strategies in the more challenging multi-domain task adaptation and dataset generalization settings. To this end, we develop \name (see Figure \ref{fig:overview}), a novel task-aware modulation approach that improves upon MuMo-MAML by: (i) evolving a meta knowledge structure $\mathcal{M}$, similar to state-of-the-art approaches; (ii) adopting a contrastive distillation strategy (with graph neural networks) to incorporate information from $\mathcal{M}$ to enrich the image embedding module; (iii) leveraging the improved image embeddings through the use of a simple task encoding scheme without any learnable parameters, unlike existing approaches that use complex task encoders; and (iv) utilizing a moving average-style update of $\mathcal{M}$ to effectively aggregate the historical experience. Interestingly, we find that, when adapting the meta-learned model to an unseen test task, \name~does not require extracting information from $\mathcal{M}$, unlike existing approaches~\citep{yao2019hierarchically,yao2020automated}. 

% \paragraph{Hierarchically Structured Meta-Learning (HSML) .} The core idea of HSML is to enhance few-shot meta-learning by explicitly inducing a task clustering step, thus enabling customization to different clusters of tasks as well as ensuring generalization among semantically related tasks. In particular, by adopting a hierarchical clustering formulation, HSML effectively performs coarse- and fine-grained categorization of heterogeneous tasks. Given a task $\mathcal{T}_i$, HSML begins by inferring a task embedding vector (a.k.a task representation), similar to TAM, using a recurrent autoencoder network. Subsequently, this task representation is augmented with information from the hierarchical knowledge structure using a soft cluster assignment strategy.

% Each node (or cluster) in the hierarchical knowledge structure contains learnable parameters (weights and biases) that are used to transform the input task representation from level $\ell-1$. The updated task representations obtained after traversing the entire hierarchy can then be leveraged to perform task-aware modulation. 

% \paragraph{Automated Relational Meta-Learning (ARML)~\citep{yao2020automated}.} While hierarchical clustering enables consistent modulation of the meta-parameters for related tasks, in practice, the design of the hierarchical structure is highly sensitive and more importantly, it relies on simple vector representations for tasks. Instead, ARML proposed to replace both task representations as well as the knowledge structure using a learnable meta-knowledge graph $\mathcal{G}$ to succinctly encode the prior knowledge as the meta-learning algorithm continues to process a sequence of tasks.


% \begin{figure*}[t]
% \centering
% \includegraphics[width=1\textwidth]{LaTeX/images/SGML.png} % Reduce the figure size so that it is slightly narrower than the column.
% \caption{An overview of the proposed approach for structure-aware meta-learning. \method~represents input few-shot tasks using prototype graphs and constructs knowledge graph hierarchies to capture task relationships as the algorithms processes a sequence of tasks. For any task $\mathcal{T}_i$, its prototype graph is augmented with relevant information from the learned knowledge structure (\textit{i.e.}, prior experience). Finally, the updated task representations are used to modulate the global meta-initialization parameters $\theta_0$ to obtain task-specific initialization $\theta_{0_i}$. }
% \label{fig:overview}
% \end{figure*}



==> CAML - Arxiv/sections/problem.tex <==

In this section, we describe the problem settings considered in this study for studying the behavior of different task-aware meta learning approaches. Figure~\ref{fig:problems} provides an overview of the formulations considered. Broadly, in few-shot classification, training tasks drawn from the distribution $p^{tr}(\mathcal{T})$ are used to learn how to adapt quickly to any of the tasks, and evaluated on previously unseen test tasks from $p^{te}(\mathcal{T})$. Common to all these formulations is that within each of the one or more datasets, the classes seen during training are completely disjoint from those seen during testing. However, the formulations vary in terms of distribution shifts and semantic disparities.
%The overarching goal in all these settings is to build models that can quickly adapt to new tasks with little data. 

\vspace{0.1in}
\noindent \textbf{A. Few-shot Task Adaptation.} In this setup, let $\mathcal{D}^{tr} = \{(\mathrm{x}_i, \mathrm{y}_i)\}_{i=1}^{|\mathcal{D}^{tr}|}$ denote the training set comprising samples $\mathrm{x}_i$ and their labels $\mathrm{y}_i$, where $\mathrm{y}_i \in \mathcal{C}^{tr}$. In other words, all samples used for training belong to one of the classes from the set $\mathcal{C}^{tr}$. The goal is to learn an adaptable model using $\mathcal{D}^{tr}$ to support learning new classes with only few examples. For evaluation, we construct a series of few-shot tasks (or episodes) and measure the model's ability to adapt to novel classes from $\mathcal{C}^{te}$ (i.e., $\mathcal{C}^{tr} \cap \mathcal{C}^{te} = \emptyset$). More specifically, each $k-$shot $N-$way test episode is represented as the tuple $\mathcal{T} = (\mathcal{S}_{\mathcal{T}}, \mathcal{Q}_{\mathcal{T}})$, where the \textit{support} set contains $k$ examples from each of the $N$ classes (selected from $\mathcal{C}^{te}$), i.e., $\mathcal{S}_{\mathcal{T}} \coloneqq \{(\mathrm{x}_1, \mathrm{y}_1), \cdots, (\mathrm{x}_{kN}, \mathrm{y}_{kN})\}$, $\mathrm{y}_i \in \{1,\cdots, N\}$, and the \textit{query} set $\mathcal{Q}_{\mathcal{T}} \coloneqq \{(\mathrm{x}^*_1, \mathrm{y}^*_1), \cdots\}$ contains different (unlabeled) examples from the same set of $N$ classes.

\vspace{0.1in}
\noindent \textbf{B. Multi-Domain Few-shot Task Adaptation.} In many practical applications, the training examples $\mathrm{x}_i \in \mathcal{D}^{tr}$ can encompass a variety of distribution shifts (e.g., variations in the data acquisition process). Hence, in this setting, we represent the training set as a composition of datasets from $M$ different domains, i.e., $\mathcal{D}^{tr} = \mathcal{D}^{tr}_1 \cup \mathcal{D}^{tr}_2 \cdots \cup \mathcal{D}^{tr}_M$, wherein all samples (regardless of the domain) belong to a 
% class chosen from a 
common family of classes $\mathcal{C}^{tr}$. The goal here is to learn to adapt to the training tasks arising from any of the $M$ domains. For evaluation, both the support and query sets for a test episode $\mathcal{T}$ are drawn from any domain $m \in \{1,\dots,M\}$, i.e., $(\mathrm{x}, \mathrm{y}) \in \mathcal{D}^{te}_m$ and the $N$ classes are picked from a disjoint set $\mathcal{C}^{te}$ similar to the previous case.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/overview.pdf}
    \caption{\textbf{Approach Overview}. An illustration of the proposed approach for task-aware meta learning.}
    \label{fig:overview}
\end{figure}

\vspace{0.1in}
\noindent \textbf{C. Few-shot Dataset Generalization.} In this challenging variant, the training set is defined as a union of $M$ different datasets $\mathcal{D}^{tr} = \mathcal{D}^{tr}_1 \cup \mathcal{D}^{tr}_2 \cdots \cup \mathcal{D}^{tr}_M$, and more importantly, it is assumed that each dataset contains examples from different sets of classes $\{\mathcal{C}^{tr}_m\}_{m=1}^M$. As a result, the goal here is to learn to adapt to completely different semantic concepts corresponding to each of the $M$ datasets. For evaluation, we construct test episodes using novel unseen classes from an entirely different dataset $\mathcal{D}_{M+1}^{te}$. Denoting the set of classes in the novel dataset as $\mathcal{C}_{M+1}^{te}$, we will study how effectively one can leverage the prior to generalize to unseen datasets.

% For a task $\mathcal{T}_i$ sampled from an underlying task distribution $P(\mathcal{T})$, we have $D^{tr}_i = {(\mathrm{x}_j, y_j) : j \in [1,N^{tr}]}$ constituting the training set, and correspondingly $D^{ts}_i$ representing the test set. The goal is to perform an $K$-way classification task, where $K$ is the number of unique labels in task $\mathcal{T}_i$. Note, while the number of classes $K$ is typically fixed across tasks, the specific classes vary across tasks. In few-shot learning settings, the number of data examples (or \textit{shots}) in each class is assumed to be very small. During the training phase, the model can access several tasks $\{\mathcal{T}_i\}$, from which it can ``learn to learn'' effectively.

% Given a base learner $f$ with initial parameters $\theta_0$, in the meta train phase, we first update $\theta_0$ using the training data $D^{tr}_i$ corresponding to the task $\mathcal{T}_i$ ,
% \begin{equation} \label{eq:1}
% \theta^*_{i} = \theta_0 - \alpha\nabla_{\theta}\mathcal{L}_{\tau_i}(f_{\theta_{0i}}),
% \end{equation}


% for each task $\tau_i$ sampled from  the meta learner $\mathcal{M}$ updates  with prior knowledge to obtain task specific initial parameters $\theta_{0i}$. The optimal task specific initial parameters $\theta^*_{i}$ are learned by minimizing the loss function $\mathcal{L}(f_{\theta_{0i}}, D^{tr}_i)$ over few gradient descent steps as shown in Equation \ref{eq:1}. To obtain the optimal initial parameters  $\theta^*_0$ and to update the meta learner with prior knowledge,  the loss $\mathcal{L}(f_{\theta^*_i}, D^{ts}_i)$  is minimized on the test dataset of task $\tau_i$ using task-specific initial parameters $\theta^*_{i}$. 

% During the training process, the parameters of base learner $f$ and the meta-learner $\mathcal{M}$ are optimized alternatively. 
     

% \begin{equation} \label{eq:2}
% \theta_0^* = \min_{\theta_0} \sum_{\tau_i \in p(\tau)} \mathcal{L}_{\tau_i}(f_{\theta^*_{i}}, D^{ts}_i)
% \end{equation}

==> CAML - Arxiv/sections/results.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Few-shot task adaptation}. Performance comparison of the proposed approach against state-of-the-art meta-learning methods. Following standard practice, we show results for $4$ different datasets from the Meta-Dataset benchmark. }
\renewcommand*{\arraystretch}{1.3}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c||c||c||c||c||c|}
  \hhline{|-||-||-||-||-||-|}
  \cellcolor[HTML]{C0C0C0}Method& 
  \cellcolor[HTML]{C0C0C0}Bird&
  \cellcolor[HTML]{C0C0C0}Texture&
  \cellcolor[HTML]{C0C0C0}Aircraft & 
  \cellcolor[HTML]{C0C0C0}Fungi & 
  \cellcolor[HTML]{C0C0C0}Average\\
%   \hhline{=::=::=::=::=::=:}
\hhline{======}
\rowcolor[HTML]{EFEFEF} \multicolumn{6}{|c|}{Number of Shots = 1} \\
\hhline{======}
  Meta-SGD~\citep{li2017meta} & 55.58 $\pm$ 1.43   & 32.38 $\pm$ 1.32   & 52.99 $\pm$ 1.36   & 41.74 $\pm$ 1.34   & 45.67\\
  
  \hhline{=::=::=::=::=::=:}
  MAML~\citep{finn2017model} &
  53.94 $\pm$ 1.45   & 31.66 $\pm$ 1.31   & 51.37 $\pm$ 1.38   & 42.12 $\pm$ 1.36   & 44.77\\
  
  \hhline{=::=::=::=::=::=:}
  MT-Net~\citep{lee2018gradient} &
  58.72 $\pm$ 1.43   & 32.80 $\pm$ 1.35   & 47.72 $\pm$ 1.46   & 43.11 $\pm$ 1.42   & 45.59\\
  
  \hhline{=::=::=::=::=::=:}
  B-MAML~\citep{yoon2018bayesian} &
   54.89 $\pm$ 1.48   & 32.53 $\pm$ 1.33   & 53.63 $\pm$ 1.37   & 42.50 $\pm$ 1.33   & 45.88\\
  
  \hhline{=::=::=::=::=::=:}
  HSML~\citep{yao2019hierarchically} &
  55.99 $\pm$ 1.41   & 32.51 $\pm$ 1.35   & 51.26 $\pm$ 1.35   & 42.86 $\pm$ 1.42   & 45.66\\
  
    \hhline{=::=::=::=::=::=:}
  MuMo-MAML~\citep{vuorio2019multimodal} &
  56.82 $\pm$ 1.49   & 33.81 $\pm$ 1.36   & 53.14 $\pm$ 1.39   & 42.22 $\pm$ 1.40   & 46.50 \\
  
  \hhline{=::=::=::=::=::=:}
  ARML~\citep{yao2020automated} &
  59.43 $\pm$ 1.46   & 33.30 $\pm$ 1.30   & 56.20 $\pm$ 1.34   & 45.85  $\pm$ 1.46 & \cellcolor[HTML]{FFDD86}48.70
  \\
  
  \hhline{=::=::=::=::=::=:}
  \textbf{Proposed} &
  59.71 $\pm$ 1.46 &
  35.47 $\pm$ 1.38 &
  57.55 $\pm$ 1.37&
  44.97 $\pm$ 1.44&
  \cellcolor[HTML]{b1e9b0}49.425\\
  
  \hhline{======}
\rowcolor[HTML]{EFEFEF} \multicolumn{6}{|c|}{Number of Shots = 5} \\
\hhline{======}

Meta-SGD~\citep{li2017meta} & 67.87 $\pm$ 0.74	  & 45.49 $\pm$ 0.68   & 66.84 $\pm$ 0.70	& 52.51 $\pm$ 0.81	 & 58.18 \\
  
  \hhline{=::=::=::=::=::=:}
  MAML~\citep{finn2017model} &
  68.52 $\pm$ 0.79	  & 44.56 $\pm$ 0.68   & 66.18 $\pm$ 0.71	& 51.85 $\pm$ 0.85	 & 57.77\\
  
  \hhline{=::=::=::=::=::=:}
  MT-Net~\citep{lee2018gradient} &
  69.22 $\pm$ 0.75	  & 46.57 $\pm$ 0.70   & 63.03 $\pm$ 0.69	& 53.49 $\pm$ 0.83	 & 58.08\\
  
  \hhline{=::=::=::=::=::=:}
  B-MAML~\citep{yoon2018bayesian} &
   69.01 $\pm$ 0.74	  & 46.06 $\pm$ 0.69   & 65.74 $\pm$ 0.67	& 52.43 $\pm$ 0.84	 & 58.31 \\
  
  \hhline{=::=::=::=::=::=:}
  HSML~\citep{yao2019hierarchically} &
  72.07 $\pm$ 0.71	  & 44.71 $\pm$ 0.66   & 64.73 $\pm$ 0.69	& 53.38 $\pm$ 0.79   & 58.65\\
  
    \hhline{=::=::=::=::=::=:}
  MuMo-MAML~\citep{vuorio2019multimodal} &
  70.49 $\pm$ 0.76	  & 45.89 $\pm$ 0.69   & 67.31 $\pm$ 0.68	& 53.96 $\pm$ 0.82	 & 59.41  \\
  
  
  \hhline{=::=::=::=::=::=:}
  ARML~\citep{yao2020automated} &
  71.97 $\pm$ 0.70	  & 47.18 $\pm$ 0.78   & 73.63 $\pm$ 0.64	& 55.23 $\pm$ 0.81  & \cellcolor[HTML]{FFDD86}62.00 \\
   
   \hhline{=::=::=::=::=::=:}
  \textbf{Proposed} &
  73.09 $\pm$ 0.73 &
  48.62 $\pm$ 0.69 &
  72.88 $\pm$ 0.64 &
  56.11 $\pm$ 0.81 &
  \cellcolor[HTML]{b1e9b0}62.675\\
  
  \hhline{|-||-||-||-||-||-|}

\end{tabular}
}
\label{table:task-shift}
\end{table*}

\begin{table*}[t]
\centering
\caption{\textbf{Multi-Domain task adaptation}. Performance comparison of ARML and \name when the meta-learners were trained using tasks from multiple domains. \name produces consistently improved generalization in all settings.}
\renewcommand*{\arraystretch}{1.3}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{|c||c||c||c||c||c|}
  \hhline{|-||-||-||-||-||-|}
  \cellcolor[HTML]{C0C0C0}Method& 
  \cellcolor[HTML]{C0C0C0}ClipArt&
  \cellcolor[HTML]{C0C0C0}InfoGraph&
  \cellcolor[HTML]{C0C0C0}Painting & 
  \cellcolor[HTML]{C0C0C0}QuickDraw & 
  \cellcolor[HTML]{C0C0C0}Average\\
    
\hhline{======}
\rowcolor[HTML]{EFEFEF} \multicolumn{6}{|c|}{Number of Shots = 1} \\
\hhline{======}

ARML~\citep{yao2020automated} &
  47.46 $\pm$ 1.48	  & 30.61 $\pm$ 1.26 & 40.26 $\pm$ 1.41	& 65.71 $\pm$ 1.33	 & \cellcolor[HTML]{FFDD86}46.01 %\cellcolor[HTML]{FFCB2F}
  \\
  
  \hhline{=::=::=::=::=::=:}
  \textbf{Proposed} &
  49.52 $\pm$ 1.47	  & 34.96 $\pm$ 1.39 & 43.98 $\pm$ 1.47	& 63.59 $\pm$ 1.40 &
  \cellcolor[HTML]{b1e9b0}48.01\\ %\cellcolor[HTML]{67FD9A}
   \hhline{======}

\rowcolor[HTML]{EFEFEF}\multicolumn{6}{|c|}{Number of Shots = 5} \\

\hhline{======}
ARML~\citep{yao2020automated} &
  66.58 $\pm$ 0.73	  & 46.19 $\pm$ 0.76  & 56.86 $\pm$ 0.72	& 83.14 $\pm$ 0.55	 & \cellcolor[HTML]{FFDD86}63.19
  \\
  \hhline{=::=::=::=::=::=:}
  \textbf{Proposed} &
  68.47 $\pm$ 0.71	  & 50.35 $\pm$ 0.75 & 60.94 $\pm$ 0.70	& 83.47 $\pm$ 0.57 &
  \cellcolor[HTML]{b1e9b0}65.80\\
  
  \hhline{|-||-||-||-||-||-|} 
\end{tabular}
}
\label{table:multi-domain}
\end{table*}

\paragraph{\textbf{Datasets}.} We consider two large-scale benchmark datasets to evaluate our proposed task-aware modulation approach under the three settings in Figure \ref{fig:problems}: \textit{(i) Meta-Dataset:} This is a widely adopted benchmark~\citep{triantafillou2019meta} for few-shot image classification and is comprised of multiple image-classification datasets. From this benchmark, we utilize six datasets for our experiments - (a) CUB-200-2011 (Bird) dataset with 200 classes; (b) describable textures dataset (Texture) with 43 classes; (c) FGVC aircraft (Aircraft) dataset with 100 classes; (d) FGVCx-fungi (Fungi) dataset with 1500 classes; (e) VGG flowers (Flower) dataset containing 102 classes; and (f) German traffic signs dataset (Traffic) with 43 classes. For training \name~as well as the baseline methods, we sampled $5$-way few-shot tasks from these datasets for $1-$ and $5-$shot training settings. In each of these datasets, we also constructed disjoint subsets of classes $\mathcal{C}^{tr}$ and $\mathcal{C}^{te}$ for training and testing respectively. For evaluation, we again construct $k$-shot $N$-way tasks from the unseen classes $\mathcal{C}^{te}$. For training and evaluation following SOTA, the images were sized $84\times84\times3$; \textit{(ii) DomainNet:} This is a popular benchmark dataset~\citep{peng2019moment} for domain adaptation and contains images from six different domains (clip-art, info-graph, painting, quick-draw, real, and sketch) belonging to $345$ classes. To ensure availability of sufficient data for creating few-shot tasks, we ignored classes which have less then 50 images and used random splits of $136$ and $39$ classes for training and evaluation.

\noindent \textbf{Experimental details:} For all our experiments we utilized a meta knowledge graph with 4 nodes each of size 128. We leverage a single layer Graph Convolutional Network (GCN) with \textit{tanh} activation for neural message passing. The base learner used a 4 layer CNN with $3\times3$ filters and a single liner classification layer. The 1-shot algorithms were trained for 50K iterations and the 5-shot experiments we trained for 40K iterations, both using a meta batch size of $4$. We utilized the Adam optimizer for the meta update step and for the inner loop, we performed 5 gradient steps using SGD.

%, represented as $\mathcal{T} = (\mathcal{S}_{\mathcal{T}}, \mathcal{Q}_{\mathcal{T}})$, where $\mathcal{S}_{\mathcal{T}}$ represents the support set contains $k$ samples from each $N$ classes and the query set contains different samples from the same set of $N$ classes.

\subsection{Findings}
\noindent \textbf{\name~is an effective protocol for task-aware modulation.} In our first experiment, we evaluated the ability of \name~to adapt to novel tasks sampled from unseen classes and compared against different gradient-based meta learning approaches on the Meta-Dataset benchmark. From the results in Table \ref{table:task-shift}, we clearly notice that approaches that leverage task-aware modulation, e.g., MuMo-MAML, HSML, ARML, \name~etc., consistently outperform vanilla meta-learning approaches such as MAML and Meta-SGD. Among existing task-aware modulation strategies, ARML has been known to produce state-of-the-art results on this benchmark\footnote{We used the official implementation from the original authors (https://github.com/huaxiuyao/ARML) to generate all results in our experimental setup. Even with the prescribed settings, we are not able to reproduce the results from their paper. A few others have also raised this issue on Github, but the authors had not responded at the time of submission.}. We find that \name~provides marginal improvements over ARML in both $1-$ and $5-$ shot training settings as shown in Table \ref{table:task-shift}. This can be attributed to the ability of \name~to capture complex task relations using the meta knowledge structure and to effectively distill relevant historical information into the embedding function. Interestingly, CAML eliminates the need for sophisticated task encoding architectures typically used by existing approaches (e.g., RNN autoencoders).

\begin{table*}[t]
\centering
\caption{\textbf{Dataset Generalization}. The evaluation is carried out using a leave-one-out protocol on the meta-dataset. We find that, \name~achieves significantly improved performance over ARML.}
\renewcommand*{\arraystretch}{1.3}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{|c||c||c||c||c||c||c||c|}
  \hhline{|-||-||-||-||-||-||-||-|}
  \cellcolor[HTML]{C0C0C0}Method& 
  \cellcolor[HTML]{C0C0C0}Bird&
  \cellcolor[HTML]{C0C0C0}Texture&
  \cellcolor[HTML]{C0C0C0}Aircraft & 
  \cellcolor[HTML]{C0C0C0}Fungi & 
  \cellcolor[HTML]{C0C0C0}Flower&
  \cellcolor[HTML]{C0C0C0}Traffic&
  \cellcolor[HTML]{C0C0C0}Average\\

  \hhline{========}
\rowcolor[HTML]{EFEFEF} \multicolumn{8}{|c|}{Number of Shots = 1} \\
\hhline{========}
  ARML~\citep{yao2020automated} &
  38.34 $\pm$ 1.35 & 
  27.13 $\pm$ 1.33 & 
  27.45 $\pm$ 1.23 & 
  32.85	$\pm$ 1.38 & 
  54.79 $\pm$ 1.35 & 
  39.36 $\pm$ 1.33 & \cellcolor[HTML]{FFDD86}36.65
  \\
  
  \hhline{=::=::=::=::=::=::=::=:}
  \textbf{Proposed} &
   40.56 $\pm$ 1.42 & 
   28.75 $\pm$ 1.33 & 
   28.41 $\pm$ 1.24 & 
   33.73 $\pm$ 1.37 & 
   57.89 $\pm$ 1.43 & 
   44.22 $\pm$ 1.39 & \cellcolor[HTML]{b1e9b0}38.93\\
   \hhline{========}

\rowcolor[HTML]{EFEFEF}\multicolumn{8}{|c|}{Number of Shots = 5} \\

\hhline{========}
ARML~\citep{yao2020automated} &
  55.48	$\pm$ 0.80&
  36.49 $\pm$ 0.64&
  36.39 $\pm$ 0.63&
  44.15	$\pm$ 0.73&
  71.80 $\pm$ 0.68&
  52.69 $\pm$ 0.66&\cellcolor[HTML]{FFDD86}49.5
  \\
  
  \hhline{=::=::=::=::=::=::=::=:}
  \textbf{Proposed} &
  58.48 $\pm$ 0.72& 
  39.78 $\pm$ 0.65& 
  39.45 $\pm$ 0.65& 
  45.26 $\pm$ 0.75& 
  73.12 $\pm$ 0.69& 
  62.18 $\pm$ 0.69& \cellcolor[HTML]{b1e9b0}53.1
  \\ 
  \hhline{|-||-||-||-||-||-||-||-|}
\end{tabular}
}
\label{table:dataset-generalization}
\end{table*}

% Furthermore, our novel contrastive training enables us to use a na\"ive task encoding scheme, thus improving the computational efficiency of our inference step. 
% However, ARML relies on a sophisticated RNN architecture for task encoding, and more importantly, requires neural message passing from the meta knowledge graph for obtaining effective task representations at test time.In contrast, 

% the embedding functions improves the expressive power of the embedding to produce rich task representation vectors infused with prior task information. Along with simplifying the aggregation strategy, \name adopts a novel moving average based update of knowledge graph with task information. This update ensures the capture of rich task specific information by the knowledge graph in contrast to ARML, which updates the knowledge graph using the gradients from the meta update step.

\noindent \textbf{\name~is consistently better in multi-domain task adaptation.} To further study the performance of \name~on heterogeneous task distributions, in this experiment, we considered DomainNet, a multi-domain benchmark. While both the training and testing tasks were drawn from the same collection of domains (ClipArt, InfoGraph, Painting, QuickDraw), we ensured that the set of classes $\mathcal{C}^{tr}$ and $\mathcal{C}^{te}$ were disjoint. In this setting, the increased complexity of the task distribution makes the modulation process more sensitive, when compared to the previous experiment. For simplicity, we compare \name~with the best performing task-aware modulation baseline, \textit{i.e.}, ARML. As shown in Table \ref{table:multi-domain}, CAML achieves performance gaps of $2\%$ and $2.6\%$ on average, in $1-$ and $5-$shot settings respectively. This clearly demonstrates the effectiveness of \name~in handling heterogeneous task distributions.
% This result stands testimony to our \name's ability to adapt to a more challenging task adaptation setting when compared to ARML by capturing domain specific information along with class specific information.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/analysis.pdf}
    \caption{\textbf{Ablations}. (a) Sensitivity of $\alpha$, $\lambda$; (b) We observe that the adaptation performance of \name~does not improve by including the meta knowledge graph (KG) during adaptation.}
    \label{fig:comp}
\end{figure*}

\noindent \textbf{\name~provides significant gains in dataset generalization.}
Finally, the dataset generalization experiment investigates the ability of \name to generalize to unseen datasets - for example utilizing the knowledge about \textit{Fungi} and \textit{Birds} to solve tasks sampled from \textit{Traffic}. The lack of apparent semantic similarity between the classes across different datasets can make this significantly harder than the previous two scenarios. However, improved performance in this problem will be of the most practical value.

In this experiment, we evaluate the generalization using a leave-one-out protocol, where we train the meta learner using $5$ datasets in Meta-Dataset and evaluate on the sixth dataset. From Table \ref{table:dataset-generalization}, we find that \name~achieves significant performance gains over ARML for all datasets and training settings. For example, on the \textit{Traffic} dataset, the performance gain is as high as $\sim5\%$ in the $1-$shot case and $\sim10\%$ in the $5-$shot case, thus establishing \name~as the best performing task-aware modulation approach. The observed performance improvements emphasize the efficacy of our meta knowledge construction process, and the expressiveness of the task representations learned by \name.

% Importantly, the performance gap between \name and ARML increases as the test task complexity increases, showing the efficacy of the moving average update of the knowledge graph adopted by \name. This improved knowledge update with current task information leads to significantly improved few-shot generalization.

\subsection{Ablations}
In this section, we briefly discuss about the behavior of \name~and the impact of different design choices. 

\noindent (i) \textbf{\textit{Choice of $\alpha$ and $\lambda$}}: Figure \ref{fig:comp}(a) illustrates the sensitivity of different choices for $\alpha$ and $\lambda$. While $\alpha$ controls the degree to which the history is retained, $\lambda$ controls the penalty for the distillation cost. These two parameters are used to trade-off generalization (to new tasks) and customization (to observed tasks) of the learner. We find that, when $\alpha$ is very low, i.e., knowledge graphs evolves slowly, using a higher $\lambda$ hurts the performance. On the other hand, for a reasonably higher $\alpha = 0.2$, the choice of $\lambda$ becomes less sensitive. In all our experiments, we used $\alpha = 0.2, \lambda=0.05$.

\noindent (ii) \textbf{\textit{Choice of feature extractor}}: CAML uses an image embedding function to create node features for the prototype graph, which is then subsequently used to generate a task representation. In the algorithm described in the main paper, this embedding module is implemented using a convolutional neural network. As discussed in the ablations (Section 5.2), we studied the impact of the choice of architecture for this module. In particular, we experimented with (i) ResNet-18 model; and (ii) a shallow CNN model (similar to MuMo-MAML), for the case of dataset generalization. As illustrated in Table \ref{table:ablation-feature_extractor}, we find that the performance gap between the two models is only $\sim 0.8\%$ on average, in terms of generalizing to unseen datasets. This behavior emphasizes the flexibility of implementing CAML in practice, wherein the proposed contrastive distillation strategy is effective with any architecture choice.

\begin{table}[t]
\centering
\caption{\textbf{Choice of architecture for the image embedding module}. We compare the performance of a shallow CNN model and ResNet-18 (used in the main paper) using the dataset generalization experiment. In each case, we show the results obtained using $1000$ test tasks for the $1-$shot setting. }
\renewcommand*{\arraystretch}{1.3}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{|c||c||c|}
  \hhline{|-||-||-|}
  \cellcolor[HTML]{C0C0C0}Dataset& 
  \cellcolor[HTML]{C0C0C0}ResNet-18&
  \cellcolor[HTML]{C0C0C0}Shallow CNN\\

  \hhline{===}
  Bird & 40.56 $\pm$ 1.42 & 38.18 $\pm$ 1.34\\
  Texture & 28.75 $\pm$ 1.33 &27.91 $\pm$ 1.33 \\
  Aircraft & 28.41 $\pm$ 1.24 &27.77 $\pm$ 1.27 \\
%   Fungi & 33.73 $\pm$ 1.37 &$\pm$ \\
%   Flower & 57.89 $\pm$ 1.43 & 53.74 $\pm$ 1.39\\
  Traffic & 44.22 $\pm$ 1.39 & 44.70 $\pm$ 1.32 \\
  \hhline{===}
  Average & 35.48 & 34.64\\
  \hhline{|-||-||-|}
\end{tabular}
}
\label{table:ablation-feature_extractor}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{Choice of task encoding scheme}. We compare the performance of a sophisticated task encoding process (RNN autoencoder) and the na\"ive average pooling strategy used in the main paper, using the dataset generalization experiment. In each case, we show the results obtained using $1000$ test tasks for the $1-$shot setting. }
\renewcommand*{\arraystretch}{1.3}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{|c||c||c|}
  \hhline{|-||-||-|}
  \cellcolor[HTML]{C0C0C0}Dataset& 
  \cellcolor[HTML]{C0C0C0}Average Pooling&
  \cellcolor[HTML]{C0C0C0}RNN Autoenc.\\

  \hhline{===}
  Bird & 40.56 $\pm$ 1.42 &40.88 $\pm$ 1.39\\
  Texture & 28.75 $\pm$ 1.33 &28.41 $\pm$ 1.28 \\
  Aircraft & 28.41 $\pm$ 1.24 &28.75 $\pm$ 1.25 \\
  Fungi & 33.73 $\pm$ 1.37 & 34.71	$\pm$ 1.38\\
  Flower & 57.89 $\pm$ 1.43 & 57.53 $\pm$  1.44\\
  Traffic & 44.22 $\pm$ 1.39 &43.44 $\pm$ 1.35\\
  \hhline{===}
  Average & 38.93 & 38.95 \\
  \hhline{|-||-||-|}
\end{tabular}
}
\label{table:ablation-feature_extractor}
\end{table}

\noindent (iii) \textbf{\textit{Choice of task encoding}}: The task encoder in CAML is used generate a compact representation for a given task, based on its prototype graph features. Though a contrastive training objective is included during training, the prototype node features from the image embedding module can be directly used for constructing task representations. In existing task-aware MAML approaches, this step has been found to be crucial and hence sophisticated task encoders are often used. For example, state-of-the-art approaches such as HSML and ARML utilize a RNN auto-encoder, wherein the latent representations from the bottleneck layer are used as the task encodings. In our paper, we argued that, through the use of inherently effective image embeddings (a result of our proposed contrastive training process), we are able to use na\"ive task encodings without any learnable parameters. To validate this claim, we re-implemented CAML using the RNN autoencoder-based task encodings and compared it against the results reported in the main paper. Similar to the previous ablation, we used the dataset generalization experiment and report results for the $1-$shot setting (see Table \ref{table:ablation-feature_extractor}). We find that the RNN autoencoder did not lead to any significant changes in performance (on average the difference was only $0.02$\%).

\noindent (iv) \textbf{\textit{Influence of using meta knowledge during adaptation}}: Though we used a simple protocol for adaptation, we also experimented a variant, where we performed knowledge infusion (using NMP) at test time. As showed in Figure \ref{fig:comp}(b), we found that this did not provide any additional performance gains, thus implying that the relevant prior information has already been effectively distilled into the embedding function. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/conv.png}
    \caption{Convergence characteristics of CAML and ARML for a dataset generalization experiment in the $1-$shot training setting.}
    \label{fig:conv}
\end{figure}

\subsection{Analysis}
\noindent \textbf{Training Behavior.} We now report the training behavior of CAML, in comparison to ARML, in terms of the accuracy metric measured using the query sets of each of the training tasks observed during every iteration of training. Figure \ref{fig:conv} shows the convergence characteristics of the two methods for the dataset generalization case, where we train the models using the following $5$ datasets. Bird, Texture, Aircraft, Fungi, Flower. As expected, the inherently large diversity in the observed tasks from the different datasets makes training of both CAML and ARML challenging. Note, these results correspond to the $1-$shot training case. From the plot, it is apparent that, CAML demonstrates improved convergence and produces higher accuracies on the query set, even in this challenging setting.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/gsp.pdf}
    \caption{Graph Signal Analysis of the task encodings from CAML (bottom) and ARML (top). For each method, we show the $2-$D TSNE embeddings of the corresponding task encodings and the graph Fourier spectra of the accuracy scores on the k-nearest neighbor graphs constructed from the task encodings ($k=5$).}
    \label{fig:gsp}
\end{figure}

\noindent \textbf{Analysis of task encodings.} In order to analyze the characteristics of the task encodings from CAML and ARML, we conducted the following analysis using tools from graph signal processing. More specifically, we first computed the set of task representations $\mathrm{Z}^{\text{CAML}}$ and $\mathrm{Z}^{\text{ARML}}$ respectively, for a set of $1000$ unseen tasks from a dataset generalization experiment (Traffic is the unseen dataset). We also obtain the few-shot classification accuracies for all $1000$ tasks using the CAML and ARML models (on the query set), which are denoted as $\mathrm{f}^{\text{CAML}}$ and $\mathrm{f}^{\text{ARML}}$. 

Our hypothesis is that if the task representations are informative, two different tasks that have similar encodings (and hence similar task characteristics) should lead to similar accuracy scores. To test this hypothesis, we construct k-nearest neighbor graphs for both CAML and ARML embeddings to obtain the graph adjacency matrices $\mathrm{G}^{\text{CAML}}$ and $\mathrm{G}^{\text{ARML}}$. Next, we computed the graph Fourier basis using the pygsp package (https://github.com/epfl-lts2/pygsp). Finally, we compute the graph Fourier transform for the function defined as the accuracy scores. The expectation is that, when the task encodings are meaningful, the resulting graph Fourier spectrum should concentrate most of the signal's energy at low-frequencies. Figure \ref{fig:gsp} illustrates the Fourier spectra obtained for results from CAML and ARML, when the number of neighbors $k$ was set to $5$. Even with such a small neighborhood size, the spectra for ARML contains non-trivial energy at even high frequencies, thus indicating that the task encodings are not  consistent with the expected classification performance. In contrast, for CAML, we notice that most of the signal energy is concentrated at low frequencies, thus justifying its improved generalization.

% \begin{enumerate}
%     \item Shallow feature extractor vs ResNet-50 \textcolor{red}{[ToDo]}
%     \item Hyperparameter analysis - Fix $\alpha$, and vary $\lambda$. Fix $\lambda$, and vary $\alpha$ \textcolor{orange}{[Partial]}
%     \item Hypothesis of not needing to use knowledge integration at test time. \textcolor{green}{[Done]}
% \end{enumerate}
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\columnwidth]{figures/sensitivity.pdf}
% \caption{Sensitivity of $\alpha$, $\lambda$.}
% \label{fig:sens}
% \end{figure}



% Meta-SGD\shortcite{li2017meta}                      & 67.87 $\pm$ 0.74	  & 45.49 $\pm$ 0.68   & 66.84 $\pm$ 0.70	& 52.51 $\pm$ 0.81	 & 58.18   & 8         \\ \hline
% MAML\shortcite{finn2017model}                         & 68.52 $\pm$ 0.79	  & 44.56 $\pm$ 0.68   & 66.18 $\pm$ 0.71	& 42.12 $\pm$ 1.36	 & 57.77   & 7           \\ \hline
% MT-Net\shortcite{lee2018gradient}                       & 69.22 $\pm$ 0.75	  & 46.57 $\pm$ 0.70   & 63.03 $\pm$ 0.69	& 53.49 $\pm$ 0.83	 & 58.08   & 6         \\ \hline
% B-MAML\shortcite{yoon2018bayesian}                       & 69.01 $\pm$ 0.74	  & 46.06 $\pm$ 0.69   & 65.74 $\pm$ 0.67	& 52.43 $\pm$ 0.84	 & 58.31   & 6.75           \\ \hline
% MuMo-MAML\shortcite{vuorio2019multimodal}                      & 70.49 $\pm$ 0.76	  & 45.89 $\pm$ 0.69   & 67.31 $\pm$ 0.68	& 53.96 $\pm$ 0.82	 & 59.41   & 4.75         \\ \hline
% HSML\shortcite{yao2019hierarchically}                         & 72.07 $\pm$ 0.71	  & 44.71 $\pm$ 0.66   & 64.73 $\pm$ 0.69	& 53.38 $\pm$ 0.79   & 58.65   & 6.75           \\ \hline
% ARML\shortcite{yao2020automated}                         & 71.97 $\pm$ 0.70	  & 47.18 $\pm$ 0.71   & \textbf{73.63 $\pm$ 0.64}	& 55.23 $\pm$ 0.81	 & 62.00   & 2.75          \\ \hline
% Ours {[}1,2,1{]}             & \textbf{74.09 $\pm$ 0.73}	  & 47.97 $\pm$ 0.68   & 73.05 $\pm$0.66 	& 56.37 $\pm$ 0.81	 & \textbf{62.87}   & \textbf{1.75}         \\ \hline
% Ours {[}1,2,2,1{]}           & 72.57 $\pm$ 0.74	  & \textbf{48.21 $\pm$ 0.67}   & 72.50 $\pm$ 0.65	& \textbf{56.39 $\pm$ 0.80}	& 62.41   & \textbf{1.75}         \\ \hline

% \end{tabular}
% \label{table:results}
% \end{table*}


% \subsection{Dataset Description}
% We consider six benchmark image datasets to construct the few-shot classification experiments: CUB-200-2011 (Bird) with 200 classes, Describable Textures Dataset (Texture) with 43 classes, FGVC of Aircraft (Aircraft) with 100 classes, FGVCx-Fungi (Fungi)) with 1500 classes, VGG Flower (Flower) with 102 classes, and the German traffic signs dataset (Traffic Signs) with 43 classes. All datasets were obtained as part of the Meta-Dataset~\citep{triantafillou2019meta}, a large-scale benchmark for evaluating meta-learning algorithms. While the first four datasets are used to train and evaluate different structure-aware meta-learning approaches, the latter two are used to test the generalization capability of the base learner to novel, unseen datasets. For training the proposed algorithm as well as the baseline methods, we sampled the few-shot tasks $\tau_i$ from each of the four datasets, wherein the training set $D_i^{tr}$ and the test set $D_i^{ts}$ contain $K$ classes with $N_k^{tr}$ shots per class. 
% % Along with increased heterogeneity, we also utilize these two dataset to investigate the ability of a trained meta-learning methods to learn tasks sampled from unseen data distribution.


% \subsection{Setup}
% We follow  the standard protocol for training and evaluating few-shot image classification approaches~\citep{yao2019hierarchically}. Similar to~\citep{finn2017model}, we utilize a simple 4 layer convolutional network as the base learner. For our embedding function $\mathcal{B}$, we use a LeNet~\citep{lecun2015lenet} model, a popular choice for image feature extraction. The aggregating RNN encoder and decoder functions are constructed using GRU\citep{chung2014empirical}. Finally, we use a single layer GCN~\citep{kipf2016semi} to implement the "message passing" function between a meta-knowledge graph and a prototype graph. As described in the previous section, all vertices and edges of each knowledge graph in the hierarchy are randomly initialized. Note that, for fair comparison, we regenerated the results for both HSML\footnote{https://github.com/huaxiuyao/HSML} and ARML\footnote{https://github.com/huaxiuyao/ARML} at our end using the publicly released codes with the same experiment setup as that of \method.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\linewidth]{LaTeX/images/4dataset_novel.pdf}
%     \caption{Knowledge graph hierarchies from \method provide improved inductive biases for generalizing the base learner to even novel unseen datasets.}
%     \label{fig:novel}
% \end{figure}

% % All the SGML models discussed in the paper were trained using Adam optimizer with 1 cycle learning rate.
% % To evaluate the ability of the our meta-learning framework we utilize 


% % and to evaluate the ability to solve tasks sampled from unseen distributions two experimental setup is designed.
% % where the training and evaluating tasks are sampled from the same data distributions, i.e. training task and evaluation tasks are sampled from one of the 6 datasets


% % We divide all datasets into meta-train, meta-validation, and meta-task classes, performing $N$-way $K$-shot classification.  \mh{models and hyperparameter description here}

% \begin{figure*}[t]
%     \centering
%     \subfloat[Impact of increasing the number of knowledge graph nodes on ARML~\citep{yao2020automated}.]{\includegraphics[width=0.9\linewidth]{LaTeX/images/4dataset_1shot_ARML.pdf}
%      \label{fig:1shot_arml}}
%      \vfill
%      \subfloat[Impact of choosing different configurations of the knowledge graph hierarchies on \method.] {\includegraphics[width=0.9\linewidth]{LaTeX/images/4dataset_1shot_SGML.pdf}
%      \label{fig:1shot_sgml}}
%     \caption{Compared to existing structure-aware meta-learning algorithms, \method~is more flexible to allow more richer configurations of knowledge structure. While the performance of ARML declines with increasing number of nodes in the knowledge graph, our approach provides higher performance gains with more complex hierarchies.}
%     \label{fig:choice}
% \end{figure*}

% \subsection{Findings}
% To illustrate the efficacy of representing historical task information in the form of knowledge graph hierarchies, we conduct extensive experiments with different knowledge structures for classification tasks. In particular, we extensively evaluate our proposed method against HSML \citep{yao2019hierarchically} and ARML \citep{yao2020automated} which are two state-of-the-art methods for using knowledge representation in meta-learning models.  To highlight the benefit of structured knowledge representations further, we also compare against several meta-learning methods that do not use have such a component, including Meta-SGD~\citep{li2017meta}, MAML~\citep{finn2017model}, MT-Net~\citep{lee2018gradient}, B-MAML~\citep{yoon2018bayesian}, and MuMo-MAML~\citep{vuorio2019multimodal}. 

% From the results in Table \ref{table:results} for both 1-shot and 5-shot experiments, we clearly see that the proposed knowledge-graph hierarchies lead to consistently superior performance over existing baselines on average across all datasets. While all structure-aware methods provide non-trivial gains over meta-learning methods that do not perform task-aware modulation, ARML was known to be the best-performing on this benchmark. In comparison, we find that, with the [1,2,2,1] configuration, \method~provides performance gains as high as $\sim 5\%$ on the Bird benchmark over ARML and a boost of $\sim2\%$ on average across all $4$ datasets. We attribute this performance boost to the use of more expressive knowledge graph hierarchies for extracting cross-task relationships. As expected, \method provides much larger improvements over HSML, $\sim 5\%$ on average with about $8.5\%$ boost on the Bird dataset. We make similar observations for the 5-shot case, where \method consistently outperforms both HSML and ARML. 

% The benefits of using a richer knowledge structure is more apparent when the trained base learner is utilized for novel, unseen datasets -- \textit{Flower} and \textit{Traffic}. From Figure \ref{fig:novel}, we observe that our proposed knowledge graph hierarchies provide better inductive biases, as reflected by the significant improvements in the generalization performance when compared to ARML. For a rigorous comparison, we show the results for several other meta-learning baselines and include the \textit{Average Rank} metric (based on relative ranking of the methods for each dataset) for a more holistic understanding of the different approaches. 

% An important challenge with any structure-aware learning algorithm is determining the appropriate complexity for the knowledge structure. For example, as showed in Figure \ref{fig:1shot_arml}(a), arbitrarily increasing the number of nodes in ARML shows a steady decline in the classification performance. In contrast, knowledge graph hierarchies enable more flexible customization of the structure by either increasing the depth (number of levels $L$) or changing the number of graphs in each level. Interestingly, from Figure \ref{fig:1shot_sgml}, we find that using configurations with larger depth leads to consistent improvements with heterogeneous task distributions.


% %  shows that increasing the number of learnable nodes in the meta graph of ARML  deteriorates the performance. On the other hand, with the increase in number of learnable nodes in \method, the performance consistently improves as illustrated in \ref{fig:1shot_sgml}. This performance gain is the result of organizing the learnable nodes into hierarchical structure of different meta-graphs which effectively utilizes the nodes to express heterogeneous task knowledge at different levels of complexity.

% % % Experiment about test on 5 and 6 training on 4 datasets.
% % We introduce an experiment to test the ability of the meta-learning algorithms to tasks sampled from unseen data-distribution.
% % We train the models on 4 dataset and 
% % We conduct an experiment where we train the meta-learning models on 




% \begin{table}[t]
% \centering
% \caption{Multi-Domain Training: 5 shot 5 way -- TBD}
% \renewcommand*{\arraystretch}{1.3}
% \begin{tabular}{|c||c||c||c||c||c|}
%   \hhline{|-||-||-||-||-||-|}
%   \cellcolor[HTML]{C0C0C0}Method& 
%   \cellcolor[HTML]{C0C0C0}ClipArt&
%   \cellcolor[HTML]{C0C0C0}InfoGraph&
%   \cellcolor[HTML]{C0C0C0}Painting & 
%   \cellcolor[HTML]{C0C0C0}QuickDraw & 
%   \cellcolor[HTML]{C0C0C0}Average\\
% %     \hhline{=::=::=::=::=::=:}
% %   MuMo-MAML &
% %   00.00 $\pm$ 00.00	  & 00.00 $\pm$ 00.00  & 00.00 $\pm$ 00.00	& 00.00 $\pm$ 00.00	 & 00.00 %\cellcolor[HTML]{FFCB2F}
% %   \\
  
%   \hhline{=::=::=::=::=::=:}
%   ARML &
%   66.58 $\pm$ 0.73	  & 46.19 $\pm$ 0.76  & 56.86 $\pm$ 0.72	& 83.14 $\pm$ 0.55	 & \cellcolor[HTML]{FFDD86}63.19 %\cellcolor[HTML]{FFCB2F}
%   \\
  
%   \hhline{=::=::=::=::=::=:}
%   \textbf{Proposed} &
%   67.01 $\pm$ 0.72	  & 48.42 $\pm$ 0.75 & 58.60 $\pm$ 0.71	& 82.04 $\pm$ 0.58 &
%   \cellcolor[HTML]{b1e9b0}64.02\\ %\cellcolor[HTML]{67FD9A}
%   \hhline{|-||-||-||-||-||-|}

% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Dataset Generalization: 5 shot 5 way -- TBD}
% \renewcommand*{\arraystretch}{1.3}
% \begin{tabular}{|c||c||c||c||c||c||c||c|}
%   \hhline{|-||-||-||-||-||-||-||-|}
%   \cellcolor[HTML]{C0C0C0}Method& 
%   \cellcolor[HTML]{C0C0C0}Bird&
%   \cellcolor[HTML]{C0C0C0}Texture&
%   \cellcolor[HTML]{C0C0C0}Aircraft & 
%   \cellcolor[HTML]{C0C0C0}Fungi & 
%   \cellcolor[HTML]{C0C0C0}Flower&
%   \cellcolor[HTML]{C0C0C0}Traffic&
%   \cellcolor[HTML]{C0C0C0}Average\\
% %   \hhline{=::=::=::=::=::=::=::=:}
% %   MuMo-MAML &
% %   00.00	  & 00.00  & 00.00 	& 00.00	 & 00.00 & 00.00 & %\cellcolor[HTML]{FFCB2F}
% %   \\
%   \hhline{=::=::=::=::=::=::=::=:}
%   ARML &
%   55.48	  & 36.49  & 36.39 	& 44.15	 & 71.80 & 52.69 &\cellcolor[HTML]{FFDD86}49.5
%   \\
  
%   \hhline{=::=::=::=::=::=::=::=:}
%   \textbf{Proposed} &
%   58.48 & 
%   39.78 & 
%   39.45 & 
%   45.26 & 
%   73.12 & 
%   62.18 & \cellcolor[HTML]{b1e9b0}53.16 \\
%   %\cellcolor[HTML]{67FD9A}
% %   \hhline{=::=::=::=::=::=::=:}
% %     {Improvement} &
% %   \cellcolor[HTML]{b1e9b0}+3.00  & \cellcolor[HTML]{b1e9b0}+3.29  & \cellcolor[HTML]{b1e9b0}+3.06 	& \cellcolor[HTML]{b1e9b0}+1.11	 & \cellcolor[HTML]{b1e9b0}+1.32 & \cellcolor[HTML]{b1e9b0}+10.19 \\
%   \hhline{|-||-||-||-||-||-||-||-|}
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Task-Shift: 5 shot 5 way}
% \renewcommand*{\arraystretch}{1.3}
% \begin{tabular}{|c||c||c||c||c||c|}
%   \hhline{|-||-||-||-||-||-|}
%   \cellcolor[HTML]{C0C0C0}Method& 
%   \cellcolor[HTML]{C0C0C0}Bird&
%   \cellcolor[HTML]{C0C0C0}Texture&
%   \cellcolor[HTML]{C0C0C0}Aircraft & 
%   \cellcolor[HTML]{C0C0C0}Fungi & 
%   \cellcolor[HTML]{C0C0C0}Average\\
%   \hhline{=::=::=::=::=::=:}
%   Meta-SGD & 67.87 $\pm$ 0.74	  & 45.49 $\pm$ 0.68   & 66.84 $\pm$ 0.70	& 52.51 $\pm$ 0.81	 & 58.18 \\
  
%   \hhline{=::=::=::=::=::=:}
%   MAML &
%   68.52 $\pm$ 0.79	  & 44.56 $\pm$ 0.68   & 66.18 $\pm$ 0.71	& 42.12 $\pm$ 1.36	 & 57.77\\
  
%   \hhline{=::=::=::=::=::=:}
%   MT-Net &
%   69.22 $\pm$ 0.75	  & 46.57 $\pm$ 0.70   & 63.03 $\pm$ 0.69	& 53.49 $\pm$ 0.83	 & 58.08\\
  
%   \hhline{=::=::=::=::=::=:}
%   B-MAML &
%   69.01 $\pm$ 0.74	  & 46.06 $\pm$ 0.69   & 65.74 $\pm$ 0.67	& 52.43 $\pm$ 0.84	 & 58.31 \\
  
%   \hhline{=::=::=::=::=::=:}
%   HSML &
%   72.07 $\pm$ 0.71	  & 44.71 $\pm$ 0.66   & 64.73 $\pm$ 0.69	& 53.38 $\pm$ 0.79   & 58.65\\
  
%     \hhline{=::=::=::=::=::=:}
%   MuMo-MAML &
%   70.49 $\pm$ 0.76	  & 45.89 $\pm$ 0.69   & 67.31 $\pm$ 0.68	& 53.96 $\pm$ 0.82	 & 59.41  \\
  
  
%   \hhline{=::=::=::=::=::=:}
%   ARML &
%   71.97 $\pm$ 0.70	  & 47.18 $\pm$ 0.78   & 73.63 $\pm$ 0.64	& 55.23 $\pm$ 0.81  & \cellcolor[HTML]{FFDD86}62.00 \\
   
%   \hhline{=::=::=::=::=::=:}
%   \textbf{Proposed} &
%   72.95 $\pm$ 0.72 &
%   48.31 $\pm$ 0.71 &
%   73.02 $\pm$ 0.64&
%   55.55 $\pm$ 0.81&
%   \cellcolor[HTML]{b1e9b0}62.46\\ %\cellcolor[HTML]{67FD9A}
%   \hhline{|-||-||-||-||-||-|}

% \end{tabular}
% \end{table}

